On Mismatched Oblivious Relaying

We consider the problem of reliable communication over a discrete memoryless channel (DMC) with the help of a relay, termed the information bottleneck (IB) channel. There is no direct link between the source and the destination, and the information flows in two hops. The first hop is a noisy channel from the source to the relay. The second hop is a noiseless but limited-capacity backhaul link from the relay to the decoder. We further assume that the relay is oblivious to the transmission codebook. We examine two mismatch scenarios. In the first setting, we assume the decoder is restricted to use some fixed decoding rule, which is mismatched to the actual channel. In the second setting, we assume that the relay is restricted to use some fixed compression metric, which is again mismatched to the statistics of the relay input. We establish bounds on the random- coding capacity of both settings, some of which are shown to be ensemble tight.

==> figures/ib/communication_diagram.tex <==
\def\dMEnc{1.5}
\def\dEncCh{4}
\def\dEncDec{4}
\def\dChRelay{3}
\def\dRelayDec{3}
\def\dDecHatM{1.5}
\begin{tikzpicture}[every text node part/.style={align=center}]
    \coordinate (M) at (0,0);
    \node[draw=black, minimum width=2cm, minimum height = 1cm] (enc) at (\dMEnc,0) {Encoder \\ $\rv{X}^n = f^{(n)}(\rv{M}) $};
    \node[draw=black, minimum width=2cm, minimum height = 1cm] (ch) at (\dMEnc+\dEncCh,0) {$\pmf{\rv{Y}| \rv{X}} $};
    \node[draw=black,  minimum height = 1cm] (relay) at (\dMEnc+\dEncCh + \dChRelay,0) {Relay \\ $\rv{W} = g^{(n)}(\rv{Y}^n)   $ \\ $\rv{W} \in [1:2^{nB}]$};


    \node[draw=black,  minimum height = 1cm] (dec) at (\dMEnc+\dEncCh + \dChRelay+\dRelayDec,0) {Decoder};
    \coordinate (hatM) at (\dMEnc+\dEncCh + \dChRelay + \dRelayDec+\dDecHatM,0);
    
    \draw[->] (M) node[left] {$\rv{M}$} -- (enc);
    \draw[->] (enc) --  node[above] {$\rv{X}^n$} (ch);
    \draw[->] (ch) --  node[above] {$\rv{Y}^n$} (relay);
    \draw[->] (relay) -- node[above] {$\rv{W}$} (dec); 
    \draw[->] (dec) -- (hatM) node[right]{$\hat{\rv{M}}$};
\end{tikzpicture}

==> figures/ib/source_coding_diagram.tex <==
\def\dXPxy{2}
\def\dPxyEnc{4}
\def\dEncDec{5}
\def\dDecZ{2}
\begin{tikzpicture}[every text node part/.style={align=center}]
    \coordinate (X) at (0,0);
    \node[draw=black, minimum width=2cm, minimum height = 1cm] (Pxy) at (\dXPxy,0) {$\pmf{\rv{X} \rv{Y}} $};
    \node[draw=black,  minimum height = 1cm] (enc) at (\dXPxy+\dPxyEnc,0) {Encoder \\ $f^{(n)}(\rv{Y}^n) \mapsto \rv{W}   $};
    \node[draw=black,  minimum height = 1cm] (dec) at (\dXPxy+\dPxyEnc+\dEncDec,0)  {Decoder \\ $g^{(n)}(\rv{W}) \mapsto \rv{Z}^n   $};
    \coordinate (Z) at (\dXPxy+\dPxyEnc+\dEncDec+\dDecZ,0);
    
    
    \draw[->] (Pxy) --  (X) node[left] {$\rv{X}^n$};
    \draw (Pxy) --  node[above] {$\rv{Y}^n$} (enc);
    \draw (enc) -- node[above]{$\rv{W} \in [1:2^{nR}]$} (dec);
    \draw (dec) -- (Z) node[right] {$\rv{Z}^n$};
\end{tikzpicture}

==> figures/mmdec/mmdec_quaternary_channel1_diagram.tex <==
\def\dNodesY{2}
\def\dNodesX{2}

\begin{tikzpicture}
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt,label=left:{$0$}] (in0) at (0,0) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt,label=left:{$1$}] (in1) at (0,\dNodesY) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt,label=left:{$2$}] (in2) at (0,2*\dNodesY) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt,label=left:{$3$}] (in3) at (0,3*\dNodesY) {};

    \node[circle,fill=black,inner sep=0pt,minimum size=3pt,label=right:{$0$}] (out0) at (\dNodesX,0) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt,label=right:{$1$}] (out1) at (\dNodesX,\dNodesY) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt,label=right:{$2$}] (out2) at (\dNodesX,2*\dNodesY) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt,label=right:{$3$}] (out3) at (\dNodesX,3*\dNodesY) {};

    \draw[->,olive,thick] (in0) -- node[above]{$1-\epsilon$} (out0);
    \draw[->,red,thick] (in0) -- node[above,sloped, xshift=-5]{$\frac{\epsilon}{2}$} (out1);
    \draw[->,red,thick] (in0) --  (out3);
    \draw[->,olive,thick] (in1) -- (out1);
    \draw[->,purple,thick] (in1) --  (out0);
    \draw[->,purple,thick] (in1) --  (out2);
    \draw[->,olive,thick] (in2) -- (out2);
    \draw[->,orange,thick] (in2) --  (out1);
    \draw[->,orange,thick] (in2) --  (out3);
    \draw[->,olive,thick] (in3) -- (out3);
    \draw[->,pink,thick] (in3) --  (out0);
    \draw[->,pink,thick] (in3) --  (out2);
\end{tikzpicture}

==> figures/mmdec/mmdec_quaternary_channel2_diagram.tex <==
\def\dNodesY{2}
\def\dNodesX{2}

\begin{tikzpicture}
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt,label=left:{$0$}] (in0) at (0,0) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt,label=left:{$1$}] (in1) at (0,\dNodesY) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt,label=left:{$2$}] (in2) at (0,2*\dNodesY) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt,label=left:{$3$}] (in3) at (0,3*\dNodesY) {};

    \node[circle,fill=black,inner sep=0pt,minimum size=3pt,label=right:{$0$}] (out0) at (\dNodesX,0) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt,label=right:{$1$}] (out1) at (\dNodesX,\dNodesY) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt,label=right:{$2$}] (out2) at (\dNodesX,2*\dNodesY) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt,label=right:{$3$}] (out3) at (\dNodesX,3*\dNodesY) {};

    \draw[->,olive,thick] (in0) -- node[above]{$1-\epsilon$} (out0);
    \draw[->,red,thick] (in0) -- node[above,sloped, xshift=-5]{$\frac{\epsilon}{3}$} (out1);
    \draw[->,red,thick] (in0) --  (out2);
    \draw[->,red,thick] (in0) --  (out3);
    \draw[->,olive,thick] (in1) -- (out1);
    \draw[->,purple,thick] (in1) --  (out0);
    \draw[->,purple,thick] (in1) --  (out2);
    \draw[->,purple,thick] (in1) --  (out3);
    \draw[->,olive,thick] (in2) -- (out2);
    \draw[->,orange,thick] (in2) --  (out1);
    \draw[->,orange,thick] (in2) --  (out3);
    \draw[->,orange,thick] (in2) --  (out0);
    \draw[->,olive,thick] (in3) -- (out3);
    \draw[->,pink,thick] (in3) --  (out0);
    \draw[->,pink,thick] (in3) --  (out1);
    \draw[->,pink,thick] (in3) --  (out2);
\end{tikzpicture}

==> figures/mmrdib/block_diagram.tex <==
\def\dMEnc{1.5}
\def\dEncCh{3}
\def\dChRelay{3}
\def\dRelayDec{4}
\def\dDecHatM{2}
\begin{tikzpicture}[every text node part/.style={align=center}]
    \coordinate (M) at (0,0);
    \node[draw=black, minimum width=2cm, minimum height = 1cm] (enc) at (\dMEnc,0) {Encoder \\ $\rv{X}^n = f^{(n)}(\rv{M}) $};
    \node[draw=black, minimum width=2cm, minimum height = 1cm] (ch) at (\dMEnc+\dEncCh,0) {$\pmf{\rv{Y}| \rv{X}} $};
    \node[draw=black,  minimum height = 1cm] (relay) at (\dMEnc+\dEncCh + \dChRelay,0) {Mismatched \\ Relay };


    \node[draw=black,  minimum height = 1cm] (dec) at (\dMEnc+\dEncCh + \dChRelay+\dRelayDec,0) {Decoder \\ $
    \max V(z^n(w)|x^n(m)) $};

    \coordinate (hatM) at (\dMEnc+\dEncCh + \dChRelay+\dRelayDec+\dDecHatM,0);

    
    \draw[->] (M) node[left] {$\rv{M}$} -- (enc);
    \draw[->] (enc) --  node[above] {$\rv{X}^n$} (ch);
    \draw[->] (ch) --  node[above] {$\rv{Y}^n$} (relay);
    \draw[->] (relay) -- node[above] {$\rv{W}$} (dec);
    \draw[->] (dec) -- (hatM) node[right]{$\hat{\rv{M}}$};
\end{tikzpicture}

==> figures/mmrscll/block_diagram.tex <==
\def\dXPxy{2}
\def\dPxyEnc{4}
\def\dEncDec{5}
\def\dDecZ{2}
\begin{tikzpicture}[every text node part/.style={align=center}]
    \coordinate (X) at (0,0);
    \node[draw=black, minimum width=2cm, minimum height = 1cm] (Pxy) at (\dXPxy,0) {$\pmf{\rv{X} \rv{Y}} $};
    \node[draw=black,  minimum height = 1cm] (enc) at (\dXPxy+\dPxyEnc,0) {Encoder \\ $f^{(n)}(\rv{Y}^n) \mapsto \rv{W}   $};
    \node[draw=black,  minimum height = 1cm] (dec) at (\dXPxy+\dPxyEnc+\dEncDec,0)  {Decoder \\ $g^{(n)}(\rv{W}) \mapsto \rv{Z}^n   $};
    \coordinate (Z) at (\dXPxy+\dPxyEnc+\dEncDec+\dDecZ,0);
    
    
    \draw[->] (Pxy) --  (X) node[left] {$\rv{X}^n$};
    \draw (Pxy) --  node[above] {$\rv{Y}^n$} (enc);
    \draw (enc) -- node[above]{$\rv{W} \in [1:2^{nR}]$} (dec);
    \draw (dec) -- (Z) node[right] {$\rv{Z}^n$};
\end{tikzpicture}

==> sections/auxiliary.tex <==
\subsection{Markov Typicality Lemma}
The following lemma will be utilized to prove that the correct messages are jointly typical with the received sequences at the decoder.

\begin{proof}
    \begin{align}
        &\Prob{\left|\pi(a,b,c | x^n,y^n,\rv{Z}^n) - \pmf{\rv{X}\rv{Y}\rv{Z}}(a,b,c) \right| > \epsilon \pmf{\rv{X}\rv{Y}\rv{Z}} (a,b,c) } \\
        &= \Prob{\left| \frac{\pi(a,b,c | x^n,y^n,\rv{Z}^n)}{\pmf{\rv{X}\rv{Y}}(a,b)} - \pmf{\rv{Z}|\rv{X}\rv{Y}}(c|a,b) \right| > \epsilon \pmf{\rv{Z}|\rv{X}\rv{Y} } (c|a,b) } \\
        &= \Prob{\left| \frac{\pi(a,b,c | x^n,y^n,\rv{Z}^n)}{\pi(a,b | x^n,y^n)} \frac{\pi(a,b| x^n,y^n)}{\pmf{\rv{X}\rv{Y}}(a,b)} - \pmf{\rv{Z}|\rv{Y}}(c|b) \right| > \epsilon \pmf{\rv{Z}|\rv{Y} } (c|b) } \\
        &= \Prob{\left| \frac{\pi(a,b,c | x^n,y^n,\rv{Z}^n)}{\pi(a,b | x^n,y^n) \pmf{\rv{Z}|\rv{Y} } (c|b) } \frac{\pi(a,b| x^n,y^n)}{\pmf{\rv{X}\rv{Y}}(a,b)} - 1 \right| > \epsilon } \\
        &\leq \Prob{\frac{\pi(a,b,c | x^n,y^n,\rv{Z}^n)}{\pi(a,b | x^n,y^n) \pmf{\rv{Z}|\rv{Y} } (c|b) } \frac{\pi(a,b| x^n,y^n)}{\pmf{\rv{X}\rv{Y}}(a,b)}  < 1- \epsilon } 
        + \Prob{\frac{\pi(a,b,c | x^n,y^n,\rv{Z}^n)}{\pi(a,b | x^n,y^n) \pmf{\rv{Z}|\rv{Y} } (c|b) } \frac{\pi(a,b| x^n,y^n)}{\pmf{\rv{X}\rv{Y}}(a,b)}  > 1+ \epsilon }\\
    \end{align}
    Since $(x^n,y^n) \in \typset{\epsilon''}{n} (\pmf{\rv{X}\rv{Y}})$, then
    \begin{equation}
        1-\epsilon'' \leq \frac{\pi(a,b| x^n,y^n)}{\pmf{\rv{X}\rv{Y}}(a,b)} \leq 1+\epsilon''.
    \end{equation}
    Thus,
    \begin{equation}
        \Prob{\frac{\pi(a,b,c | x^n,y^n,\rv{Z}^n)}{\pi(a,b | x^n,y^n) \pmf{\rv{Z}|\rv{Y} } (c|b) } \frac{\pi(a,b| x^n,y^n)}{\pmf{\rv{X}\rv{Y}}(a,b)}  < 1- \epsilon } 
        \leq 
        \Prob{\frac{\pi(a,b,c | x^n,y^n,\rv{Z}^n)}{\pi(a,b | x^n,y^n)  }   < \frac{1-\epsilon}{1-\epsilon''} \cdot \pmf{\rv{Z}|\rv{Y} } (c|b) } 
    \end{equation}
    and
    \begin{equation}
        \Prob{\frac{\pi(a,b,c | x^n,y^n,\rv{Z}^n)}{\pi(a,b | x^n,y^n) \pmf{\rv{Z}|\rv{Y} } (c|b) } 
        \frac{\pi(a,b| x^n,y^n)}{\pmf{\rv{X}\rv{Y}}(a,b)}  > 1+\epsilon } 
        \leq 
        \Prob{\frac{\pi(a,b,c | x^n,y^n,\rv{Z}^n)}{\pi(a,b | x^n,y^n)  }   < \frac{1+\epsilon}{1+\epsilon''} \cdot \pmf{\rv{Z}|\rv{Y} } (c|b) } 
    \end{equation}
    Now, note that
    \begin{align}
        n \pi(a,b,c | x^n,y^n, z^n)
        &= \sum_{i=1}^n \indicator {x_i=a, y_i=b, z_i = c } \\
        &= \sum_{k \colon x_k=a,y_k=b} \indicator {z_k = c }.
    \end{align}
    Thus,
    \begin{align}
        n \Exp{\pi(a,b,c | x^n,y^n, z^n)}
        &=  \sum_{k \colon x_k=a,y_k=b} \Exp{ \indicator {\rv{Z}_k = c }} \\
        &=  \sum_{k \colon x_k=a,y_k=b} \pmf{\rv{Z}|\rv{Y}}(c|b)
    \end{align}
\end{proof}

==> sections/comm_problem_formulation.tex <==
Consider the oblivious communication system diagram illustrated in \autoref{fig:ib_communication_diagram}.
\begin{figure}[b]
    \centering
    \input{./figures/ib/communication_diagram}
    \caption{Oblivious Communication System}
    \label{fig:ib_communication_diagram}
\end{figure}

Let $\{\rv{X}_i,\rv{Y}_i \}_{i=1}^n = (\rv{X}^n,\rv{Y}^n)$ be a sequence of $n$ independent, identically distributed random variables distributed according to the joint \acrshort{pmf} $\pmf{\rv{X}\rv{Y}} = \pmf{\rv{X}} \pmf{\rv{Y}|\rv{X}}$.

A $(2^{nR}, 2^{nB},n)$ code for the DM-IB consists of
\begin{itemize}
    \item a message set $\set{M} = [1:2^{nR}]$,
    \item a representation set $\set{W} = [1:2^{nB}]$,
    \item an encoder that assigns a codeword $x^n(m)$ to each message $m \in \set{M}$,
    \item an relay encoder that assigns an index $w \in \set{W}$ to each received sequence $ y^n \in \set{Y}^n$, and
    \item a decoder that assigns an estimate $\hat{m}$ or an error message e to each received representation $w \in \set{W}$.
\end{itemize}
The channel is memoryless in the sense that the current received symbol $\rv{Y}_i$ and the the message and past symbols $(m,\rv{X}^{i-1},\rv{Y}^{i-1})$ are conditionaly independent given the current transmitted symbol $\rv{X}_i$.

We assume that the message $\rv{M}$ is uniformly distributed over $\set{M}$. The average probability of error is defined as $P_e^{(n)} = \Prob{\hat{\rv{M}} \neq \rv{M}}$. A rate $R$ is said to be achievable for the DM-IB if there exists a sequence of $(2^{nR},2^{nB},n)$ codes such that $\lim_{n \rightarrow \infty } P_e^{(n)} = 0$.

\begin{theorem}
    The capacity of the discrete memoryless channel with oblivious relay and rate limited frnothaul link $B$ is given by
    \begin{equation}
        \begin{aligned}
            &C(B) =
            && \max_{\pmf{\rv{Z}|\rv{Y}}} 
            && I(\rv{X};\rv{Z}) \\
            &&& \text{subject to}
            && I(\rv{Y};\rv{Z}) \leq B,
        \end{aligned}
    \end{equation}
    where $|\set{Z}| \leq |\set{Y}|+1$.
\end{theorem}

\subsection{Proof of the Converse}
We denote $\rv{Z}_i \triangleq (\rv{W},\rv{Y}^{i-1}) $. With this notation established, we have the following string
of inequalities:
\begin{align}
    nB
    &\geq H(\rv{W}) \\
    &\geq I(\rv{W};\rv{Y}^n) \\
    &= H(\rv{Y}^n) - H(\rv{Y}^n|\rv{W}) \\
    &= \sum_{i=1}^n H(\rv{Y}_i) - H(\rv{Y}_i|\rv{W},\rv{Y}^{i-1}) \\
    &= \sum_{i=1}^n H(\rv{Y}_i) -  H(\rv{Y}_i|\rv{Z}_i) \\
    &= \sum_{i=1}^n I(\rv{Y}_i;\rv{Z}_i) \\
    &= n \sum_{i=1}^n \frac{1}{n} I(\rv{Y}_\rv{Q};\rv{Z}_\rv{Q}|\rv{Q}=i) \\
    &= n I(\rv{Y}_{\rv{Q}};\rv{Z}_{\rv{Q}}| \rv{Q})\\
    &= n I(\rv{Y}_{\rv{Q}};\rv{Z}_{\rv{Q}}, \rv{Q}) -  n I(\rv{Y}_{\rv{Q}};\rv{Q}) \\
    &= n I(\rv{Y}_{\rv{Q}};\rv{Z}_{\rv{Q}}, \rv{Q})\\
    &= n I(\rv{Y};\rv{Z}).
\end{align}
Also,
\begin{align}
    nR
    &= H(\rv{M}) \\
    &= I(\rv{M};\rv{W}) + H(\rv{M}|\rv{W}) \\
    &\leq I(\rv{X}^n;\rv{W}) + n \epsilon_n \\
    &= I(\rv{X}^n, \rv{Y}^n;\rv{W}) - I(\rv{Y}^n;\rv{W}|\rv{X}^n) + n \epsilon_n \\
    &= I(\rv{Y}^n;\rv{W}) -H(\rv{Y}^n|\rv{X}^n) +  H(\rv{Y}^n|\rv{W},\rv{X}^n) + n \epsilon_n \\
    &\leq nB -H(\rv{Y}^n|\rv{X}^n) +  H(\rv{Y}^n|\rv{W},\rv{X}^n) + n \epsilon_n
\end{align}
Note that,
\begin{align}
    H(\rv{Y}^n|\rv{X}^n) -  H(\rv{Y}^n|\rv{W},\rv{X}^n)
    &= \sum_{i=1}^n H(\rv{Y}_i|\rv{X}_i) - H(\rv{Y}_i|\rv{W},\rv{X}^n,\rv{Y}^{i-1}) \\
    &\geq \sum_{i=1}^n H(\rv{Y}_i|\rv{X}_i) - H(\rv{Y}_i|\rv{Z}_i,\rv{X}_i) \\
    &= n [H(\rv{Y}|\rv{X})-H(\rv{Y}_{\rv{Q}}|\rv{X}_{\rv{Q}},\rv{Z}_{\rv{Q}},\rv{Q})] \\
    &= n [H(\rv{Y}|\rv{X})-H(\rv{Y}|\rv{X},\rv{Z})] \\
    &= nI(\rv{Y};\rv{Z}|\rv{X})
\end{align}
Thus,
\begin{align}
    R &\leq [B-I(\rv{Y};\rv{Z}|\rv{X})]^+, \\
    B &\geq I(\rv{Y};\rv{Z}).
\end{align}

\subsection{Proof of Achievability}
We use random coding.
\paragraph{Transmitter's codebook generation.}  Fix the \acrshort{pmf} $\pmf{\rv{X}}$. Randomly and independently generate $2^{nR}$ sequences $x^n(m)$, $m \in [1:2^{nR}]$, each according to $ \pmf{\rv{X}^n} (x^n) = \prod_{i=1}^n \pmf{\rv{X}}(x_i)$. These sequences constitute the transmitter's codebook $\set{C}_{T}$, which is revealed to the transmitter and the receiver but not the relay before transmission commences.

\paragraph{Relay's codebook generation.} Fix the conditional \acrshort{pmf} $\pmf{\rv{Z}|\rv{Y}}$. Randomly and independently generate $2^{nB}$ sequences $z^n(w)$, $w \in [1:2^{nB}]$, each according to $ \pmf{\rv{Z}^n} (z^n) =  \prod_{i=1}^n \pmf{\rv{Z}}(z_i)$. These sequences constitute the relay's codebook $\set{C}_{R}$, which is revealed to both the relay and the receiver but not the transmitter before transmission takes place.


\paragraph{Encoding.} To send message $m$, the transmitter sends $x^n(m)$.

\paragraph{Relay encoding.} Upon observing $y^n$, the relay finds an index $w$ such that $(y^n,z^n(w)) \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}\rv{Z}})$. If there is more than one such index, it selects one of them uniformly at random. If there is no such index, it select an index from $[1:2^{nB}]$ uniformly at random. The relay conveys the index $w$ to the decoder.

\paragraph{Decoding}
Upon receiving $w$ from the relay, the decoder finds the unique index $\hat{m}$ such that $(x^n(\hat{m}),z^n(w)) \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{X}\rv{Z}})$ for some $\hat{m} \in [1:2^{nR}]$. If there is none or more than one such message $\hat{m}$, the decoder declares an error e.

\paragraph{Analysis of the probability of error at the relay.}
Assume without loss of generality that $\rv{M}=1$ was sent and $\rv{W}$ was chosen by the relay's encoder. Define the ``encoding error" event
\begin{equation}
    \tilde{\event{E}} = \{ (\rv{Y}^n,\rv{Z}^n(\rv{W})) \notin \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}\rv{Z}}) \},
\end{equation}
let $\epsilon'' < \epsilon'$ and consider the events
\begin{align}
    \tilde{\event{E}}_1 &= \{ \rv{Y}^n \notin \set{T}_{\epsilon''}^{(n)}(\pmf{\rv{Y}}) \},\\
    \tilde{\event{E}}_2 &= \{ \rv{Y}^n \in \set{T}_{\epsilon''}^{(n)}(\pmf{\rv{Y}}), (\rv{Y}^n,\rv{Z}^n(w)) \notin \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}\rv{Z}}) \text{ for all } w\in [1:2^{nB}] \}.
\end{align}
Then by the union of events bound,
\begin{equation}
    \Prob{\tilde{\event{E}}} = \Prob{\tilde{\event{E}}_1 \cup \tilde{\event{E}}_2} \leq \Prob{\tilde{\event{E}}_1} + \Prob{\tilde{\event{E}}_2}.
\end{equation}
We bound each term. Since $\pmf{\rv{Y}^n}(y^n) = \prod_{i=1}^n \pmf{\rv{Y}
} (y_i)$, by the \acrshort{lln}, the first term $\Prob{\tilde{\event{E}}_1}$ tends to zero as $n \rightarrow \infty $. Consider the second term
\begin{align}
    \Prob{\tilde{\event{E}}_2}
    &= \Prob{\rv{Y}^n \in \set{T}_{\epsilon''}^{(n)}(\pmf{\rv{Y}}), (\rv{Y}^n,\rv{Z}^n(w)) \notin \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}\rv{Z}}) \text{ for all } w\in [1:2^{nB}]} \\
    &= \sum_{y^n \in \set{T}_{\epsilon''}^{(n)}(\pmf{\rv{Y}})} \pmf{\rv{Y}^n} (y^n) \Prob{(\rv{Y}^n,\rv{Z}^n(w)) \notin \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}\rv{Z}}) \text{ for all } w\in [1:2^{nB}] | \rv{Y}^n=y^n} \\
    &= \sum_{y^n \in \set{T}_{\epsilon''}^{(n)}(\pmf{\rv{Y}})} \pmf{\rv{Y}^n} (y^n)\Prob{(y^n,\rv{Z}^n(w)) \notin \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}\rv{Z}}) \text{ for all } w\in [1:2^{nB}] | \rv{Y}^n=y^n} \\
    &= \sum_{y^n \in \set{T}_{\epsilon''}^{(n)}(\pmf{\rv{Y}})} \pmf{\rv{Y}^n} (y^n)\prod_{w=1}^{2^{nB}} \Prob{(y^n,\rv{Z}^n(w)) \notin \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}\rv{Z}}) } \\
    &= \sum_{y^n \in \set{T}_{\epsilon''}^{(n)}(\pmf{\rv{Y}})} \pmf{\rv{Y}^n} (y^n) \left( \Prob{(y^n,\rv{Z}^n(1)) \notin \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}\rv{Z}}) } \right)^{2^{nB}}.
\end{align}
Since $y^n \in \set{T}_{\epsilon''}^{(n)}(\pmf{\rv{Y}})$ and $\rv{Z}^n(1) \sim \prod_{i=1}^n \pmf{\rv{Z}} (z_i)$ it follows by the joint typicality lemma \cite[Ch. 2.5]{gamal2011} that for $n$ sufficiently large
\begin{equation}
    \Prob{(y^n,\rv{Z}^n(1)) \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}\rv{Z}}) }  \geq 2^{-n(I(\rv{Y};\rv{Z}) + \delta(\epsilon'))},
\end{equation}
where $\delta(\epsilon')$ tends to zero as $\epsilon' \rightarrow 0$. Since $(1-x)^k \leq e^{-kx}$ for $x \in [0,1]$ and $k>0$, we have
\begin{align}
    \sum_{y^n \in \set{T}_{\epsilon''}^{(n)}(\pmf{\rv{Y}})} \pmf{\rv{Y}^n} (y^n) \left( \Prob{(y^n,\rv{Z}^n(1)) \notin \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}\rv{Z}}) } \right)^{2^{nB}}
    & \leq  \left(1 - 2^{-n(I(\rv{Y};\rv{Z}) + \delta(\epsilon'))} \right)^{2^{nB}} \\
    & \leq  e^{-2^{-n(I(\rv{Y};\rv{Z})-B + \delta(\epsilon'))}}
\end{align}
which tends to zero as $n \rightarrow \infty$ if $B > I(\rv{Y};\rv{Z}) + \delta(\epsilon')$.

\paragraph{Analysis of the probability of error at the decoder.}
Assume without loss of generality that $\rv{M}=1$ was sent and $\rv{W}$ was chosen by the relay's encoder. 
The decoder makes an error iff one or both of the following events occur:
\begin{align}
    \set{E}_1 &= \{ (\rv{X}^n(1),\rv{Z}^n(\rv{W}) )\notin \set{T}_{\epsilon}^{(n)}(\pmf{\rv{X} \rv{Z}}) \},\\
    \set{E}_2 &= \{ (\rv{X}^n(m),\rv{Z}^n(\rv{W}) )\in \set{T}_{\epsilon}^{(n)}(\pmf{\rv{X} \rv{Z}}) \text{ for some } m \neq 1 \}.
\end{align}
Then by the union of events bound,
\begin{equation}
    \Prob{\event{E}} = \Prob{\event{E}_1 \cup \event{E}_2} \leq \Prob{\event{E}_1} + \Prob{\event{E}_2}.
\end{equation}
We bound each term. Consider the complement of the first term.
\begin{align}
    \Prob{\set{E}_1^c}
    &= \Prob{(\rv{X}^n(1),\rv{Z}^n(\rv{W}) )\in \set{T}_{\epsilon}^{(n)}(\pmf{\rv{X} \rv{Z}})} \\
    &\geq \Prob{(\rv{X}^n(1),\rv{Y}^n,\rv{Z}^n(\rv{W}) )\in \set{T}_{\epsilon}^{(n)}(\pmf{\rv{X} \rv{Y} \rv{Z}})}.
\end{align}
Thus, by the Markov Lemma \cite[Lemma 12.1]{gamal2011}, 
$\lim_{n\rightarrow \infty} \Prob{\event{E}_1} = 0$.

Consider the second term
\begin{align}
    \Prob{\event{E}_2}
    &= \Prob{(\rv{X}^n(m),\rv{Z}^n(\rv{W}) )\in \set{T}_{\epsilon}^{(n)}(\pmf{\rv{X} \rv{Z}}) \text{ for some } m \neq 1} \\
    &\leq \sum_{m=2}^{2^{nR}} \Prob{(\rv{X}^n(m),\rv{Z}^n(\rv{W}) )\in \set{T}_{\epsilon}^{(n)}(\pmf{\rv{X} \rv{Z}}) } 
\end{align}
The summation argument can be bounded from below as
\begin{align}
    \Prob{(\rv{X}^n(m),\rv{Z}^n(\rv{W}) )\in \set{T}_{\epsilon}^{(n)}(\pmf{\rv{X} \rv{Z}}) } 
    &= \sum_{(x^n,z^n) \in \set{T}_{\epsilon}^{(n)}(\pmf{\rv{X} \rv{Z}}) } \pmf{\rv{X}^n \rv{Z}^n} (x^n,z^n) \\
    &= \sum_{(x^n,z^n) \in \set{T}_{\epsilon}^{(n)}(\pmf{\rv{X} \rv{Z}}) } \pmf{\rv{X}^n } (x^n) \pmf{ \rv{Z}^n} (z^n) \\
    &\leq \sum_{(x^n,z^n) \in \set{T}_{\epsilon}^{(n)}(\pmf{\rv{X} \rv{Z}}) } 2^{-n(H(\rv{X})-\delta(\epsilon))}2^{-n(H(\rv{Z})-\delta(\epsilon))} \\
    &\leq 2^{n(H(\rv{X},\rv{Z}) + \delta(\epsilon))} 2^{-n(H(\rv{X})-\delta(\epsilon))}2^{-n(H(\rv{Z})-\delta(\epsilon))} \\
    &= 2^{-n(I(\rv{X};\rv{Z})-\delta(\epsilon))}
\end{align}
Therefore,
\begin{equation}
    \Prob{\event{E}_2} \leq 2^{n(R-I(\rv{X};\rv{Z})+\delta(\epsilon))}
\end{equation}
which tends to zero as $n \rightarrow \infty$ if $R < I(\rv{X};\rv{Z}) - \delta(\epsilon)$.
Finally taking $\epsilon \rightarrow 0$ completes the proof.

==> sections/compound/compound_achievability_proof.tex <==
We use random coding. Let $\epsilon' < \epsilon$. Fix a \acrshort{pmf} $\pmf{\rv{X}}$.
% and a conditional \acrshort{pmf} $\pmf{\rv{Z}|\rv{Y}}$, which induce the marginal \acrshort{pmf}s   $\pmf{\rv{Y}}(y) = \sum_{x \in \set{X}} \pmf{\rv{Y}|\rv{X}}(y|x)  \pmf{\rv{X}} (x)$ and $\pmf{\rv{Z}}(z) = \sum_{y \in \set{Y}} \pmf{\rv{Z}|\rv{Y}}(z|y) \pmf{\rv{Y}}(y)$.
\paragraph{Transmitter's Codebook Generation and Encoding}
Generate codebook $ \set{C} \{ x^n(m) \} $, $m \in [1:2^{nR}]$ according to the procedure described in App. \ref{appendix:generic_random_coding} with $\pmf{\rv{X}}$, rate $R$ and $n$.
The codebook is revealed to the encoder and the decoder but not the relay.
The encoding procedure is as described in App. \ref{appendix:direct_encoding}.

\paragraph{Relay's Codebook Generation}
Let $\pmf{\rv{Y}_s}(y) \triangleq \pmf{\rv{Y}|\rv{S}}(y|s) =  \sum_{x \in \set{X}} \pmf{\rv{Y} |\rv{X}\rv{S}}(y|x,s) $.
For every $s \in \set{S}$, fix the conditional \acrshort{pmf} $\pmf{\rv{Z}|\rv{Y}}^{(s)} (z|y) $. This conditional \acrshort{pmf} induces a marginal $\acrshort{pmf}$ on $\set{Z}$, i.e., $\pmf{\rv{Z}_{s}}(z) \triangleq \pmf{\rv{Z}|\rv{S}} (z|s) = \sum_{y \in \set{Y}} \pmf{\rv{Z}|\rv{Y}\rv{S}} (z|y,s) $.
Randomly and independently generate $2^{nB}$ sequences $z_s^n(w)$, $w \in [1:2^{nB}]$, each according to $ \pmf{\rv{Z}_s^n} (z^n) = \prod_{i=1}^n \pmf{\rv{Z}_s}(z_i)$. These sequences constitute the relay's codebook $\set{C}_s$ for every $s \in \set{S}$. The codebook is revealed to the relay and the decoder but not to the transmitter.


\paragraph{Relay Encoding}
Upon observing $y^n$, the relay finds an index $\hat{w} \in [1:2^{nB}]$  such that 
\begin{equation}
    \left( y^n, z_s^n(\hat{w}) \right) \in \typset{\epsilon'}{n}(\pmf{\rv{Y}_s\rv{Z}}).
\end{equation}
If there is more than one such index, it select one of them uniformly at random. If there is no such index, it selects an index from $[1:2^{nB}]$ uniformly at random. The relay conveys the selected index $\hat{w}$ to the decoder. It also conveys the index $s$ based on which the compression at the relay was done.
\hl{There might be some difficulty here since $\pmf{\rv{Y}}$ depends on $s$. We should assume that the relay can learn the $\pmf{\rv{Y}_s}$, since the relay can learn the state from a relatively short training sequence as implies }\cite[Remark 7.1]{gamal2011}.

\paragraph{Decoding}
Once having $\hat{w}$, the receiver finds a unique message $\hat{m}$ such that
\begin{equation}
    \left(x^n(\hat{m}), z^n(\hat{w}) \right) \in \typset{\epsilon}{n}(\pmf{\rv{X}\rv{Z}_s}) \text{ for some } s \in \set{S}.
\end{equation}
If there is none or more than one such message -- it declares an error event $\event{E}$.

\paragraph{Analysis of the probability of error at the relay}
Let $\epsilon'' < \epsilon'$ and $W$ denote the compression index chosen by the encoder at the relay. Since $\pmf{\rv{Y}_s^n}(y^n) = \prod_{i=1}^n \pmf{\rv{Y}_s}(y_i)$, then by the \acrshort{lln} 
\begin{equation}
    \lim_{n\rightarrow \infty} \Prob{\rv{Y}_s^n \in \typset{\epsilon''}{n}(\pmf{\rv{Y}})}  = 1.
\end{equation}
Furthermore, $\rv{Z}^n(w)$, $w \in [1:2^{nB}]$, are random sequences independent of each other and $\rv{Y}^n$, distributed according to $\pmf{\rv{Z}^n(w)}(z^n) = \prod_{i=1}^n \pmf{\rv{Z}}(z_i)$. Thus, by the Covering Lemma \cite[Lemma 3.3]{gamal2011}, there exists $\delta(\epsilon')$ that tends to zero as $\epsilon' \rightarrow 0$ such that
\begin{equation}
    \lim_{n\rightarrow \infty} \Prob{\left( \rv{Y}^n, \rv{Z}^n(\rv{W}) \right) \notin \typset{\epsilon'}{n}(\pmf{\rv{Y}_s\rv{Z}})} =0,
\end{equation}
 if 
 \begin{equation}
     B > I(\rv{Y}_s;\rv{Z}) + \delta(\epsilon').
 \end{equation}
 The last condition should hold for every $ s \in \set{S}$, therefore
 \begin{equation}
     \max_{s \in \set{S}} I(\rv{Y}_s;\rv{Z}) + \delta(\epsilon') < B.
 \end{equation}
\paragraph{Analysis of the probability of error at the decoder.}
Assume without loss of generality that $\rv{M} = 1$  is sent. The decoder makes an error \acrshort{iff} one or both of the following events occur:
\begin{align}
    \event{E}_1 &\triangleq \left\{ \left( \rv{X}^n(1), \rv{Z}_s^n(W) \right) \notin \typset{\epsilon}{n}(\pmf{\rv{X}\rv{Z}_s}) \text{ for all } s \in \set{S} \right\}, \\
    \event{E}_2 &\triangleq \left\{ \left( \rv{X}^n(m), \rv{Z}^n(W) \right) \in \typset{\epsilon}{n}(\pmf{\rv{X}\rv{Z}_s} ) \text{ for some } m \in [2:2^{nR}], s \in \set{S} \right\}.
\end{align}
Then by the union of events bound,
\begin{equation}
    \Prob{\event{E}} = \Prob{\event{E}_1 \cup \event{E}_2} \leq \Prob{\event{E}_1} + \Prob{\event{E}_2}.
\end{equation}
We bound each term. Consider the first term,
Since $\pmf{\rv{X}^n(1)\rv{Y}^n}(x^n,y^n) = \prod_{i=1}^n \pmf{\rv{X}\rv{Y}} (x_i,y_i)$, $\left( \rv{X}^n(1),\rv{Y}^n \right) \in \typset{\epsilon}{n}(\pmf{\rv{X}\rv{Y}})$ and $\rv{Z}^n (\rv{W})\sim \pmf{\rv{Z}^n|\rv{Y}^n}$, by Markov Lemma \cite[Lemma 12.1]{gamal2011}, the first term also goes to zero as $n\rightarrow \infty$.

Consider the second term. Using the fact that for every $m \neq 1$ the pair $(\rv{X}^n(m),\rv{Z}_s^n(W))$ distributed according to $\pmf{\rv{X}^n(m)\rv{Z}_s^n(W)}(x^n,z^n) = \prod_{i=1}^n \pmf{\rv{X}} (x_i) \pmf{\rv{Z}_s} (z_i)$, by the Packing Lemma \cite[Lemma 3.1]{gamal2011}, for each $s \in \set{S}$, there exists $\delta(\epsilon)$ that tends to zero as $\epsilon \rightarrow 0$ such that 
\begin{equation}
    \lim_{n \rightarrow \infty} \Prob{\rv{X}^n(m),\rv{Z}_s^n(W)) \in \typset{\epsilon}{n}(\pmf{\rv{X}\rv{Z}_s} \text{for some } m \in [2:2^{nR}] } = 0
\end{equation}
if
\begin{equation}
    R < I(\rv{X};\rv{Z}_s) - \delta(\epsilon).
\end{equation}
Hence, by the union of events bound,
\begin{align}
    \Prob{\event{E}_2} 
    &=
    \Prob{\rv{X}^n(m),\rv{Z}_s^n(W)) \in \typset{\epsilon}{n}(\pmf{\rv{X}\rv{Z}_s} \text{for some } m \in [2:2^{nR}], s \in \set{S} } \\
    &\leq |\set{S}| \max_{s \in \set{S}}  \Prob{\rv{X}^n(m),\rv{Z}_s^n(W)) \in \typset{\epsilon}{n}(\pmf{\rv{X}\rv{Z}_s} \text{for some } m \in [2:2^{nR}]} \\
\end{align}
which tends to zero as $n \rightarrow \infty$ if $ R < I(\rv{X};\rv{Z}_s) - \delta(\epsilon) $ for all $s\in \set{S}$, or equivalently, 
\begin{equation}
    R < \min_{s \in \set{S}} I(\rv{X};\rv{Z}_s) - \delta(\epsilon).
\end{equation}

==> sections/definitions/ib.tex <==
Let $\rv{X} \rightarrow \rv{Y} \rightarrow \rv{Z} $ be a Markov chain with fixed $\pmf{\rv{X}\rv{Y}}$. The \acrfull{ib} problem is defined using the following optimization problem:
\begin{equation}
    \begin{aligned}
    & I(C)  =
    && \max_{\pmf{\rv{Z}|\rv{Y}}} 
    && I(\rv{X};\rv{Z}) \\
    &&& \text{subject to}
    && I(\rv{Y};\rv{Z}) \leq C.
    \end{aligned}
\end{equation}

Evidently, $I(C)$ is an achievable rate under oblivious operation (no decoding at the relay). The non-oblivious classical rate that upper bounds this is the cut-set bound:
\begin{equation}
    I(R) \leq \min \{ I(\rv{X};\rv{Y}),C \}
\end{equation}
Communication=wise that means: decode the message at the relay $\rv{Y}$ and send what you can over the fronthaul link C.


==> sections/definitions/mmib.tex <==
Consider now the mismatched case, when the transmitter uses
random coding generated with distribution $\pmf{\rv{X}}$.
The mismatch is that the relay plans everything with
a mismatched distribution, that is not the real $\pmf{\rv{Y}|\rv{X}}$,
but some other one $\pmfQ{\rv{Y}|\rv{X}}$ (seems realistic, as discussed
to assume that $\pmf{\rv{Y}} = \pmfQ{\rv{Y}}$, that is the output distribution
is the same). Evidently now the mismatched bottleneck relates
to $\pmfQ{\rv{Z}|\rv{Y}}$, which maximizes $I(\rv{X};\rv{Z})$, under $\pmf{\rv{X}} \pmfQ{\rv{Y}|\rv{X}} \pmfQ{\rv{Z}|\rv{Y}}$,
with $I(\rv{Y};\rv{Z}) = C$. Evidently $\pmfQ{\rv{Z}|\rv{Y}}$ is not the best for $\pmf{\rv{Y}|\rv{X}}$ and denote then the degraded mismatched bottleneck by $ I_{MM}(\rv{X};\rv{Z})$ (MM stands for
mismatched).

Note that because of the random coding used by the transmitter
(who knows neither $\pmf{\rv{Y}|\rv{X}}$ nor $\pmfQ{\rv{Y}|\rv{X}}$, the rate that can be decoded equals the classical Csiszar and Korner (1981) and by Hui (1983)
bound (no need for what Anelia has described, as it is well known that
random coding is NOT optimal under mismatch) and the optimality under
random coding regime of this classical Csiszar-Korner-Hui bound is 
demonstrated in:

N. Merhav, G. Kaplan, A. Lapidoth and S. Shamai (Shitz),
"On Information Rates for Mismatched Decoders," IEEE Trans. Inform. 
Theory,
Vol. 40, No. 6, pp. 1953-1967, November 1994.

Let this mismatch rate be denoted $ I_{MM}(\rv{X};\rv{Z})$. Note that now
it is not true that:
\begin{equation}
    I_{MM}(\rv{X};\rv{Z}) \leq \min \{I_{MM}(\rv{X};\rv{Y}),C \}.
\end{equation}
We now explain the reasoning for the above inequality. Assume that the relay does knows the codebook but he applies a mismatched decoding metric. In such case, the codebook rate is defined by the mismatched virtual channel between the transmitter and the relay. But,assume that the relay applies partial decode-compress-and-forward, in such case the decoder at the destination, can use the compressed undecoded information to decoded additional bits.

Thus different examples are of interest here, and more it be
good to to examine the optimal non-oblivious relay processing
that be a combination of mismatched decode-and-forward, and
mismatched compress-and-forward. I wonder whether time sharing
(where also C is properly shared, as the constraint C is just
on average) could be declared optimal, or indeed superposition
coding is required.

A very nice and timely problem, and we have ALL tools available
(unlike the classical mismatched capacity which, as Anelia described, is 
yet open).

==> sections/generic.tex <==
\subsection{Generic Codebook Generation}
\input{sections/generic/codebook}

\subsection{Generic Encoding}
\input{sections/generic/encoding}

\subsection{Generic Compression}
\input{sections/generic/compression}

\subsection{Generic Compression Probability Error}
\input{sections/generic/compression_error}

==> sections/generic/codebook.tex <==
% \subsubsection{Generic Random Coding} 
\label{appendix:generic_random_coding}
\begin{itemize}
    \item Input: $\pmf{\rv{X}}$, rate $R$ and $n$.
    \item Randomly and independently generate $2^{nR}$ sequences $x^n(m)$, $m\in [1:2^{nR}]$, each according to $\pmf{\rv{X}^n} (x^n) = \prod_{i=1}^n \pmf{\rv{X}}(x_i)$. 
Those sequences constitute the transmitter's codebook. 
\end{itemize}



==> sections/generic/compression.tex <==
% \subsubsection{Direct Compression}
\label{appendix:direct_compression}
\begin{itemize}
    \item Input: Codebook $\set{C} = \{z^n(w)\}_{w=1}^{2^{nB}}$, source sequence $y^n$, and a joint distribution $\pmf{\rv{Y}\rv{Z}}$.
    \item Upon observing $y^n$, the relay finds an index $W \in [1:2^{nB}]$  such that 
    \begin{equation}
        \left( y^n,z^n(W) \right) \in \typset{\epsilon'}{n}(\pmf{\rv{Y}\rv{Z}}).
    \end{equation}
    If there is more than one such index, it select one of them uniformly at random. If there is no such index, it selects an index from $[1:2^{nB}]$ uniformly at random. The relay conveys the selected index $W$ to the decoder.
\end{itemize}


==> sections/generic/compression_error.tex <==
% \subsubsection{Direct Compression Error}
\label{appendix:direct_compression_error}
\begin{itemize}
    \item Input: Codebook $\set{C} = \{z^n(w)\}_{w=1}^{2^{nB}}$, \acrshort{iid} source sequence $y^n$, and a joint distribution $\pmf{\rv{Y}\rv{Z}}$.
    \item Let $\epsilon'' < \epsilon'$ and $W$ denote the compression index chosen by the encoder at the relay. Since $\pmf{\rv{Y}^n}(y^n) = \prod_{i=1}^n \pmf{\rv{Y}}(y_i)$, then by the \acrshort{lln} 
\begin{equation}
    \lim_{n\rightarrow \infty} \Prob{\rv{Y}^n \in \typset{\epsilon''}{n}(\pmf{\rv{Y}})}  = 1.
\end{equation}
Furthermore, $ \{ \rv{Z}^n(w) | w \in [1:2^{nB}] 
\} $, are random sequences independent of each other and $\rv{Y}^n$, distributed according to $\pmf{\rv{Z}^n(w)}(z^n) = \prod_{i=1}^n \pmf{\rv{Z}}(z_i)$. Thus, by the Covering Lemma \cite[Lemma 3.3]{gamal2011}, there exists $\delta(\epsilon')$ that tends to zero as $\epsilon' \rightarrow 0$ such that
\begin{equation}
    \lim_{n\rightarrow \infty} \Prob{\left( \rv{Y}^n, \rv{Z}^n(\rv{W}) \right) \notin \typset{\epsilon'}{n}(\pmf{\rv{Y}\rv{Z}})} =0,
\end{equation}
 if 
 \begin{equation}
     B > I(\rv{Y};\rv{Z}) + \delta(\epsilon').
 \end{equation}

\end{itemize}


==> sections/generic/encoding.tex <==
% \subsubsection{Direct Encoding}
\label{appendix:direct_encoding}
\begin{itemize}
    \item Input: Codebook $\set{C} = \{x^n(m)\}_{m=1}^{2^{nR}}$ and message to transmit $M$.
    \item To send message $M \in [1:2^{nR}]$, transmitter sends $x^n(M)$.
\end{itemize}

==> sections/ibcsi/ibcsi_decoder_decoding_relay_achievability_proof.tex <==
\paragraph{Transmitter's Codebook Generation}
Randomly and independently generate $2^{nR'}$ sequences $u^n(m')$, $m' \in [1:2^{nR'}]$, each according to $\pmf{\rv{U}^n} (u^n) = \prod_{i=1}^n \pmf{\rv{U}}(u_i)$. For each $m' \in [1:2^{nR'}]$, randomly and conditionally independently generate $2^{nR''}$ sequences $x^n(m',m'')$, $m'' \in [1:2^{nR''}]$, each according to $\prod_{i=1}^n \pmf{\rv{X}|\rv{U}}(x_i|u_i(m'))$.
Those sequences constitute the transmitter's codebook. The codebook is revealed to the encoder and the decoder but not the relay.
\begin{remark}
    This is a superposition coding technique as described in \cite[Ch. 5.3.1]{gamal2011}.
\end{remark}

\paragraph{Relay's Compression Codebook Generation}
For every $m' \in [1:2^{nR'}]$, randomly and independently generate $2^{nB'}$ sequences $z^n(m',w)$, $w \in [1:2^{nB'}]$, each according to $ \pmf{\rv{Z}^n|\rv{U}^n} (z^n|u^n) = \prod_{i=1}^n \pmf{\rv{Z}|\rv{U}}(z_i|u_i)$. These sequences constitute the relay's codebook. The codebook is revealed to the relay and the decoder but not to the transmitter.

\paragraph{Encoding}
To send message $m = (m',m'') \in [1:2^{nR}]$, transmitter sends $x^n(m',m'')$.

\paragraph{Relay Decoding}
Upon observing $y^n$, the relay finds an index $\hat{m}' \in [1:2^{nR'}]$  such that 
\begin{equation}
    \left( u^n(\hat{m}'),y^n \right) \in \typset{\epsilon'}{n}(\pmf{\rv{U}\rv{Y}}).
\end{equation}
If there is no such index, or there is more than one such index, the relay declares decoding error event $\event{E}'$.

\paragraph{Relay Compression}
Upon observing $y^n$ and decoding $\rv{u}^n(\hat{m}')$, the relay finds an index $\hat{w} \in [1:2^{nB'}]$  such that 
\begin{equation}
    \left( u^n(\hat{m}'),y^n, z^n(\hat{w}) \right) \in \typset{\epsilon'}{n}(\pmf{\rv{U}\rv{Y} \rv{Z}}).
\end{equation}
If there is more than one such index, it select one of them uniformly at random. If there is no such index, it selects an index from $[1:2^{nB'}]$ uniformly at random. 

The relay conveys the decoded ``cloud center" (see \cite[Ch. 5.3.1]{gamal2011}) $\hat{m}'$ and the selected compression index $\hat{w}$ to the decoder.

\paragraph{Decoding}
Once having $(\hat{m}',w)$, and observing $s^n$, the receiver finds a unique index $\hat{m}''$ such that
\begin{equation}
    \left(u^n(\hat{m}'),x^n(\hat{m}',\hat{m}''),s^n, z^n(\hat{w}) \right) \in \typset{\epsilon}{n} (\pmf{\rv{U} \rv{X} \rv{S} \rv{Z}}).
\end{equation}
If there is none or more than one such message -- it declares an error event $\event{E}$.

\paragraph{Analysis of the probability of decoding error at the relay}
Assume without loss of generality that $(\rv{M}',\rv{M}'') = 1$  is sent. The decoder makes an error \acrshort{iff} one or both of the following events occur:
\begin{align}
    \event{E}_1' &\triangleq \left\{ \left( \rv{U}^n(1), \rv{Y}^n \right) \notin \typset{\epsilon}{n}(\pmf{\rv{U}\rv{Y}}) \right\}, \\
    \event{E}_2' &\triangleq \left\{ \left( \rv{U}^n(1), \rv{Y}^n \right) \in \typset{\epsilon''}{n}(\pmf{\rv{U}  \rv{Y}} ) \text{ for some } m' \in [2:2^{nR'}] \right\}.
\end{align}
Then by the union of events bound,
\begin{equation}
    \Prob{\event{E}'} = \Prob{\event{E}_1' \cup \event{E}_2'} \leq \Prob{\event{E}_1'} + \Prob{\event{E}_2'}.
\end{equation}
We bound each term. Consider the first term,
Since
\begin{align}
    \pmf{\rv{U}^n(1) \rv{Y}^n}(u^n(1),y^n) 
    &= \sum_{m'' \in [1:2^{nR''}]} \pmf{\rv{U}^n(1) \rv{X}^n(1,m') \rv{Y}^n}(u^n(1),x^n(1,m''),y^n) \\
    &= \sum_{m'' \in [1:2^{nR''}]} \prod_{i=1}^n  \pmf{\rv{U}}(u_i) \pmf{\rv{X}|\rv{U}}(x_i(1,m'')|u_i(1)) \pmf{\rv{Y}|\rv{X}}(y_i|x_i(1,m'')) \\
    &= \prod_{i=1}^n \pmf{\rv{X} \rv{S}\rv{Y}} (x_i,s_i,y_i)
\end{align}
thus by the \acrshort{lln}, the first term $\Prob{\event{E}_1'}$ tends to zero as $n\rightarrow \infty$.

Consider the second term. Using the fact that for every $m' \neq 1$ the pair $(\rv{U}^n(m'), \rv{Y}^n)$ distributed according to $\pmf{\rv{U}^n(m') \rv{Y}^n }(u^n(m'),y^n) = \prod_{i=1}^n \pmf{\rv{U}} (u_i(m')) \pmf{\rv{Y}}(y_i) $, by the Packing Lemma \cite[Lemma 3.1]{gamal2011},  there exists $\delta(\epsilon'')$ that tends to zero as $\epsilon'' \rightarrow 0$ such that 
\begin{equation}
    \lim_{n \rightarrow \infty} \Prob{\rv{U}^n(m'),\rv{Y}^n) \in \typset{\epsilon''}{n}(\pmf{\rv{U} \rv{Y} }) \text{for some } m' \in [2:2^{nR'}] } = 0
\end{equation}
if
\begin{equation}
    R' < I(\rv{U};\rv{Y}) - \delta(\epsilon'').
\end{equation}

\paragraph{Analysis of the probability of compression error at the relay}
Let $\epsilon''' < \epsilon'$ and $W$ denote the compression index chosen by the encoder at the relay. Since $\pmf{\rv{Y}^n}(y^n) = \prod_{i=1}^n \pmf{\rv{Y}}(y_i)$, then by the \acrshort{lln} 
\begin{equation}
    \lim_{n\rightarrow \infty} \Prob{\rv{Y}^n \in \typset{\epsilon'''}{n}(\pmf{\rv{Y}})}  = 1.
\end{equation}
Furthermore, $\rv{Z}^n(m',w)$, $m' \in [1:2^{nR}]$, $w \in [1:2^{nB'}]$, are random sequences independent of each other and $\rv{Y}^n$, distributed according to $\pmf{\rv{Z}^n(m',w)|\rv{U}^n(m')}(z^n(m',w)|u^n(m')) = \prod_{i=1}^n \pmf{\rv{Z}|\rv{U}}(z_i(m',w)|u_i(m'))$. Thus, by the Covering Lemma \cite[Lemma 3.3]{gamal2011}, there exists $\delta(\epsilon')$ that tends to zero as $\epsilon' \rightarrow 0$ such that
\begin{equation}
    \lim_{n\rightarrow \infty} \Prob{\left( \rv{U}^n(1), \rv{Y}^n, \rv{Z}^n(1,\rv{W}) \right) \notin \typset{\epsilon'}{n}(\pmf{\rv{U}\rv{Y}\rv{Z}})} =0,
\end{equation}
 if 
 \begin{equation}
     B'  > I(\rv{Y};\rv{Z}|\rv{U}) + \delta(\epsilon').
 \end{equation}

\paragraph{Analysis of the probability of error at the destination decoder.}
Assume without loss of generality that $(\rv{M}',\rv{M}'') = (1,1)$  is sent and the pair $(1,W)$ was received from the relay. The decoder at the destination makes an error \acrshort{iff} one or both of the following events occur:
\begin{align}
    \event{E}_1 &\triangleq \left\{ \left( \rv{U}^n(1),\rv{X}^n(1,1), \rv{S}^n, \rv{Z}^n(1,W) \right) \notin \typset{\epsilon}{n} (\pmf{\rv{U}\rv{X}\rv{S} \rv{Z}})\right\}, \\
    \event{E}_2 &\triangleq \left\{ \left( \rv{U}^n(1),\rv{X}^n(1,m''), \rv{S}^n, \rv{Z}^n(1,W) \right) \in \typset{\epsilon}{n} (\pmf{\rv{U}\rv{X}\rv{S} \rv{Z}}) \text{ for some } m'' \in [2:2^{nR''}] \right\}.
\end{align}
Then by the union of events bound,
\begin{equation}
    \Prob{\event{E}} = \Prob{\event{E}_1 \cup \event{E}_2} \leq \Prob{\event{E}_1} + \Prob{\event{E}_2}.
\end{equation}
We bound each term. Consider the complement of the first term,
\begin{align}
    \Prob{\event{E}_1^c}
    &= \Prob{\left( \rv{U}^n(1), \rv{X}^n(1,1), \rv{S}^n, \rv{Z}^n(1,W) \right) \in \typset{\epsilon}{n}(\pmf{\rv{U}\rv{X}\rv{S} \rv{Z}})} \\
    &\geq \Prob{\left( \rv{U}^n(1), \rv{X}^n(1,1), \rv{S}^n, \rv{Y}^n, \rv{Z}^n(1,W) \right) \in \typset{\epsilon}{n}(\pmf{\rv{U}\rv{X}\rv{S} \rv{Y}\rv{Z}})} .
\end{align}
Since $\left( \rv{X}^n(1),\rv{Y}^n \right) \in \typset{\epsilon}{n}(\pmf{\rv{X}\rv{Y}})$ and $\rv{Z}^n (\rv{W})\sim \pmf{\rv{Z}^n|\rv{Y}^n}$, by Markov Lemma \cite[Lemma 12.1]{gamal2011}, the last term also goes to $1$ as $n\rightarrow \infty$.
Therefore, $\Prob{\event{E}_1}$ tends to zero as $n$ tends to infinity.

Consider the second term. Using the fact that for every $m'' \neq 1$ the quadruple $ \left( \rv{U}^n(1),\rv{X}^n(1,m''), \rv{S}^n, \rv{Z}^n(1,W) \right)$ distributed according to $\pmf{\rv{U}^n(1),\rv{X}^n(1,m''), \rv{S}^n, \rv{Z}^n(W)}(u^n(1),x^n(1,m''), s^n, z^n(1,W)) = \prod_{i=1}^n \pmf{\rv{U} \rv{X}} (u_i,x_i) \pmf{\rv{S}}(s_i) \pmf{\rv{Z}} (z_i)$, utilizing Packing Lemma \cite[Lemma 3.1]{gamal2011}, there exists $\delta(\epsilon)$ that tends to zero as $\epsilon \rightarrow 0 $ such that
$\Prob{\event{E}_2}$ tends to zero as $ n \rightarrow \infty $ if
\begin{equation}
    R'' < I(\rv{X};\rv{S},\rv{Z}|\rv{U})  - \delta(\epsilon) = I(\rv{X};\rv{Z}|\rv{U},\rv{S})  - \delta(\epsilon)  .
\end{equation}

Finally, taking $\epsilon$, $\epsilon'$, and $\epsilon''$ to zero completes the proof of the theorem.

==> sections/ibcsi/ibcsi_decoder_oblivious_relay_achievability_proof.tex <==
Let $\pmf{\rv{Y}}(y) \triangleq   \sum_{(x,s) \in \set{X} \times \set{Y}} \pmf{\rv{Y} |\rv{X}\rv{S}}(y|x,s) \pmf{\rv{X}}(x) \pmf{\rv{S}}(s)$.
Fix the conditional \acrshort{pmf} $\pmf{\rv{Z}|\rv{Y}} (z|y) $. This conditional \acrshort{pmf} induces a marginal $\acrshort{pmf}$ on $\set{Z}$, i.e., $\pmf{\rv{Z}}(z) \triangleq  \sum_{y \in \set{Y}} \pmf{\rv{Z}|\rv{Y}} (z|y) \pmf{\rv{Y}}(y) $.

\paragraph{Transmitter's Codebook Generation and Encoding}
Generate codebook $ \set{C} \{ x^n(m) \} $, $m \in [1:2^{nR}]$ according to the procedure described in App. \ref{appendix:generic_random_coding} with $\pmf{\rv{X}}$, rate $R$ and $n$.
The codebook is revealed to the encoder and the decoder but not the relay.
The encoding procedure is as described in App. \ref{appendix:direct_encoding}.

\paragraph{Relay's Codebook Generation and Compression}
Generate codebook $ \set{C}_R \{ z^n(w) \} $, $w \in [1:2^{nB}]$ according to the procedure described in App. \ref{appendix:generic_random_coding} with $\pmf{\rv{Z}}$, rate $B$ and $n$.
The codebook is revealed to the relay and the decoder but not to the transmitter. The compression is according to App. \ref{appendix:direct_compression} with $\set{C}_R$, rate $B$, the sequence $y^n$ at the output of the channel,  joint \acrshort{pmf} $\pmf{\rv{Y}\rv{Z}}$, and output index $w$ sent to the decoder. 
Using standard direct compression analysis as described in App. \ref{appendix:direct_compression_error}, such $w$ exists if
\begin{equation}
     B > I(\rv{Y};\rv{Z}) + \delta(\epsilon').
 \end{equation}

\paragraph{Decoding}
Once having $\hat{w}$ and observing $s^n$, the receiver finds a unique message $\hat{m}$ such that
\begin{equation}
    \left(x^n(\hat{m}), s^n, z^n(\hat{w}) \right) \in \typset{\epsilon}{n}(\pmf{\rv{X} \rv{S}\rv{Z}}) .
\end{equation}
If there is none or more than one such message -- it declares an error event $\event{E}$.

\paragraph{Analysis of the probability of error at the relay}
Let $\epsilon'' < \epsilon'$ and $W$ denote the compression index chosen by the encoder at the relay. Since $\pmf{\rv{Y}^n}(y^n) = \prod_{i=1}^n \pmf{\rv{Y}}(y_i)$, then by the \acrshort{lln} 
\begin{equation}
    \lim_{n\rightarrow \infty} \Prob{\rv{Y}^n \in \typset{\epsilon''}{n}(\pmf{\rv{Y}})}  = 1.
\end{equation}
Furthermore, $\rv{Z}^n(w)$, $w \in [1:2^{nB}]$, are random sequences independent of each other and $\rv{Y}^n$, distributed according to $\pmf{\rv{Z}^n(w)}(z^n) = \prod_{i=1}^n \pmf{\rv{Z}}(z_i)$. Thus, by the Covering Lemma \cite[Lemma 3.3]{gamal2011}, there exists $\delta(\epsilon')$ that tends to zero as $\epsilon' \rightarrow 0$ such that
\begin{equation}
    \lim_{n\rightarrow \infty} \Prob{\left( \rv{Y}^n, \rv{Z}^n(\rv{W}) \right) \notin \typset{\epsilon'}{n}(\pmf{\rv{Y} \rv{Z}})} =0,
\end{equation}
 if 
 \begin{equation}
     B > I(\rv{Y};\rv{Z}) + \delta(\epsilon').
 \end{equation}
\paragraph{Analysis of the probability of error at the decoder.}
Assume without loss of generality that $\rv{M} = 1$  is sent. The decoder makes an error \acrshort{iff} one or both of the following events occur:
\begin{align}
    \event{E}_1 &\triangleq \left\{ \left( \rv{X}^n(1), \rv{S}^n, \rv{Z}^n(W) \right) \notin \typset{\epsilon}{n}(\pmf{\rv{X}\rv{Z}}) \right\}, \\
    \event{E}_2 &\triangleq \left\{ \left( \rv{X}^n(m), \rv{S}^n \rv{Z}^n(W) \right) \in \typset{\epsilon}{n}(\pmf{\rv{X} \rv{S} \rv{Z}} ) \text{ for some } m \in [2:2^{nR}] \right\}.
\end{align}
Then by the union of events bound,
\begin{equation}
    \Prob{\event{E}} = \Prob{\event{E}_1 \cup \event{E}_2} \leq \Prob{\event{E}_1} + \Prob{\event{E}_2}.
\end{equation}
We bound each term. Consider the first term,
Since $\pmf{\rv{X}^n(1) \rv{S}^n \rv{Y}^n}(x^n,s^n,y^n) = \prod_{i=1}^n \pmf{\rv{X} \rv{S}\rv{Y}} (x_i,s_i,y_i)$, $\left( \rv{X}^n(1),\rv{S}^n, \rv{Y}^n \right) \in \typset{\epsilon}{n}(\pmf{\rv{X} \rv{S} \rv{Y}})$ and $\rv{Z}^n (\rv{W})\sim \pmf{\rv{Z}^n|\rv{Y}^n}$, by Markov Lemma \cite[Lemma 12.1]{gamal2011}, the first term also goes to zero as $n\rightarrow \infty$.

Consider the second term. Using the fact that for every $m \neq 1$ the pair $(\rv{X}^n(m), \rv{S}^n, \rv{Z}^n(W))$ distributed according to $\pmf{\rv{X}^n(m) \rv{S}^n \rv{Z}^n(W)}(x^n,s^n,z^n) = \prod_{i=1}^n \pmf{\rv{X}} (x_i) \pmf{\rv{S}}(s_i) \pmf{\rv{Z}_s} (z_i)$, by the Packing Lemma \cite[Lemma 3.1]{gamal2011},  there exists $\delta(\epsilon)$ that tends to zero as $\epsilon \rightarrow 0$ such that 
\begin{equation}
    \lim_{n \rightarrow \infty} \Prob{\rv{X}^n(m),\rv{S}^n, \rv{Z}^n(W)) \in \typset{\epsilon}{n}(\pmf{\rv{X} \rv{S} \rv{Z}} \text{for some } m \in [2:2^{nR}] } = 0
\end{equation}
if
\begin{equation}
    R < I(\rv{X};\rv{S}, \rv{Z}) - \delta(\epsilon) =  I(\rv{X};\rv{Z}|\rv{S}) - \delta(\epsilon).
\end{equation}


==> sections/mismatched_decoder.tex <==
Consider the channel coding problem for the \acrshort{dmc} with a mismatched decoder model $(\set{X}, \pmf{\rv{Y}|\rv{X}}, V(y|x), \set{Y})$ that consists of a finite input set (or alphabet) $\set{X}$, a finite output set $\set{Y}$, a collection of conditional \acrshort{pmf}s on $\set{Y}$ for every $x \in \set{X}$, and a mismatched decoding metric $V(y|x)$. Thus, if an input symbol $x \in \set{X}$ is transmitted, the probability of receiving an output symbol $y \in \set{Y}$ is $\pmf{\rv{Y}|\rv{X}} (y|x)$. The channel is stationary and memoryless.

A $(2^{nR},n)$ code for the \acrshort{dmc} $\pmf{\rv{Y}|\rv{X}}$ with mismathed decoder consists of
\begin{itemize}
    \item a message set $[1:2^{nR}]$,
    \item an encoding function (encoder) that assigns a codeword $x^n(m)$ to each message $m \in [1:2^{nR}]$, and
    \item a decoding function (decode) that assigns an estimate $\hat{m} \in [1:2^{nR}]$ according to the decoding metric $V(y|x)$ to each received sequence $y^n$ as follows:
    \begin{equation}
        \hat{m} = \argmax_{m \in [1:2^{nR}]} \ln V(y^n|x^n(m)) 
        = \argmax_{m \in [1:2^{nR}]} \sum_{i=1}^n \ln V(y_i|x_i(m))
    \end{equation}
    We sometimes denote the decoding metric $a_{xy} \triangleq \ln V(y|x)$.
\end{itemize}
\begin{theorem}
    A rate $R$ is achievable if
    \begin{equation}
        R \leq \max_{\pmf{\rv{X}}} I'(\rv{X};\rv{Y})
    \end{equation}
    where
    \begin{equation}
        I(\rv{X};\rv{Y}) = \sum_{x \in \set{X}} \sum_{y \in \set{y}} \pmf{\rv{X}}(x) f(y|x) \ln \frac{f(y|x)}{\sum_{x' \in \set{X}} \pmf{\rv{X}}(x') f(y|x') }
    \end{equation}
    denote the mutual information for some \acrshort{dmc} $f = \{f(x,y)\}$ with an input \acrshort{pmf} $\pmf{\rv{X}}$. Let
    \begin{equation}
        I'(\rv{X};\rv{Y}) = \min_{f} I(\rv{X};\rv{Y})
    \end{equation}
    where the minimization is over all channels $f$ satisfying
    \begin{equation}
        \sum_{x\in \set{X}} \pmf{\rv{X}} (x) f(y|x)
        = \sum_{x \in \set{X}} \pmf{\rv{X}}(x) W(y|x) \triangleq q(y) \quad \forall y \in \set{Y}
    \end{equation}
    and
    \begin{equation}
        \sum_{x\in \set{X}} \sum_{y\in \set{Y}} \pmf{\rv{X}}(x) f(y|x) \ln V(y|x)
        \geq \sum_{x\in \set{X}} \sum_{y\in \set{Y}} \pmf{\rv{X}}(x) W(y|x) \ln V(y|x)
        \triangleq -D.
    \end{equation}
\end{theorem}

\subsection{Proof of Achievability}
\paragraph{Codebook generation.} We use random coding. Fix the \acrshort{pmf} $\pmf{\rv{X}}$. Randomly and independently generate $2^{nR}$ sequences $x^n(m)$, $m \in [1:2^{nR}]$, each according to $ \pmf{\rv{X}^n}(x^n) = \prod_{i=1}^n \pmf{\rv{X}}(x_i)$. The generated sequences consitute the codebook $\set{C}$. The chosen codebook $\set{C}$ is revealed to both the encoder and the decoder before transmission commences.

\paragraph{Encoding.} To send message $m$, the encoder transmits $x^n(m)$.

\paragraph{Decoding}
The decoder finds the unique index $\hat{m}$ such that $(x^n(\hat{m}),y^n ) \in \set{T}_{\epsilon,+}^{(n)}$ for some $\hat{m} \in [1:2^{nR}]$, where
\begin{equation}
    \set{T}_{\epsilon,+}^{(n)}
    = \left\{
        (x^n,y^n) : \sum_{x,y} \left[\pmf{\rv{X}\rv{Y}}(x,y) - \pmf{\bv{x}\bv{y}}(x,y) \right] a_{xy} \leq \epsilon ,
    \right\}
\end{equation}
otherwise -- if there is none or more than one such message -- it declares an error e.
\paragraph{Analysis of the probability of error.}
Assume without loss of generality that $\rv{M}=1$ was sent. The decoder makes an error \acrshort{iff} one ore more of the following events occur:
\begin{align}
    \set{E}_1 &= \{ (\rv{X}^n(1), \rv{Y}^n) \notin \set{T}_{\epsilon ,+}^{(n)} \},\\
    \set{E}_2 &= \{ (\rv{X}^n(m), \rv{Y}^n) \in \set{T}_{\epsilon, + }^{(n)} \text{ for some } m \in [2:2^{nR}] \}.
\end{align}
Then by the union of events bound,
\begin{equation}
    \Prob{\event{E}} = \Prob{\event{E}_1 \cup \event{E}_2} \leq  \Prob{\event{E}_1 } + \Prob{\event{E}_2}.
\end{equation}
We bound each term. Applying Sanov's theorem on the first term we have
\begin{equation}
    \Prob{\event{E}_1}
    \leq (n+1)^{|\set{X}| \cdot |\set{Y}|} 2^{-n \kld{\pmf{}^*}{\pmf{\rv{X}\rv{Y}}}},
\end{equation}
where
\begin{equation}
    \kld{\pmf{}^*}{\pmf{\rv{X}\rv{Y}}} = \min_{\pmf{} \notin \set{T}_{\epsilon+}^{(n)}} \kld{\pmf{}}{\pmf{\rv{X}\rv{Y}}}.
\end{equation}
Note that $\pmf{\rv{X}\rv{Y}} \in \set{T}_{\epsilon,+}^{(n)}$, therefore $\kld{\pmf{}^*}{\pmf{\rv{X}\rv{Y}}} > 0$ and
\begin{equation}
    \lim_{n \rightarrow \infty} \Prob{\event{E}_1} = 0.
\end{equation}
Next consider the second term
\begin{align}
    \Prob{\event{E}_2}
    &= \Prob{(\rv{X}^n(m), \rv{Y}^n) \in \set{T}_{\epsilon, + }^{(n)} \text{ for some } m \in [2:2^{nR}] } \\
    &\leq \sum_{m=2}^{2^{nR}} \Prob{(\rv{X}^n(m), \rv{Y}^n) \in \set{T}_{\epsilon, + }^{(n)}  }.
\end{align}
Since for $m\neq 1$, $\pmf{\rv{X}^n(m)\rv{Y}^n} (x^n,y^n) = \prod_{i=1}^n \pmf{\rv{X}}(x_i) \pmf{\rv{Y}} (y_i)$, utilizing Sanov's theorem, we have
\begin{equation}
    \Prob{(\rv{X}^n(m), \rv{Y}^n) \in \set{T}_{\epsilon, + }^{(n)} }
    \leq (n+1)^{|\set{X}|\cdot |\set{Y}|} 2^{-n \kld{\pmf{}^*}{\pmf{\rv{X}} \pmf{\rv{Y}}}}  
\end{equation}
where
\begin{equation}
    \kld{\pmf{}^*}{\pmf{\rv{X}} \pmf{\rv{Y}}} = \min_{\pmf{} \in \set{T}_{\epsilon+}^{(n)}} \kld{\pmf{}}{\pmf{\rv{X}} \pmf{\rv{Y}}} = I'(\rv{X};\rv{Y})
\end{equation}
where 
\begin{equation}
    I'(\rv{X};\rv{Y}) = \min_{f \in \set{T}_{\epsilon,+}} \kld{f}{\pmf{\rv{X}} \pmf{\rv{Y}}}.
\end{equation}
Hence, $\Prob{\event{E}_2}$ tends to $0$ as $n\rightarrow \infty$ if $ R < I'(\rv{X};\rv{Y})$.


\subsection{Proof of the Converse}
We assume random coding.
Fix $\epsilon > 0$, and let $\typset{\epsilon}{n}(\pmf{\rv{X}})$ and $\typset{\epsilon}{n}(\pmf{\rv{Y}})$ denote the $\epsilon$--typical sets associated with the input and output marginals, respectively. Similarly, fix $\delta > 0$, and let 
\begin{equation}
    \typset{\delta ^-}{n} \triangleq \left\{ (x^n,y^n) \colon \log V(y^n|x^n) \leq n(-D+\delta) \right\}.
\end{equation}
Assume without loss of generality that message $\rv{M}=1$ was sent. The average probability of correct message decoding can be upper bounded as follows:
\begin{align}
    1 - \Bar{P_e}
    &= \Prob{V(y^n|x^n(m)) < V(y^n|x^n(1)) \text{ for all } m \in [2:2^{nR}] } \\
    &\leq \Prob{V(y^n|x^n(m)) < V(y^n|x^n(1)) \text{ for all } m \in [2:2^{nR}], (x^n(1),y^n) \in \typset{\delta^-}{n}, y^n \in \typset{\epsilon}{n}(\pmf{\rv{Y}})}  \\
    & + \Prob{y^n \notin \typset{\epsilon}{n}(\pmf{\rv{Y}}) } + \Prob{(x^n(1),y^n) \notin \typset{\delta^-}{n}}.
\end{align}
Now, the two last terms on the rightmost side vanish as $n \rightarrow \infty$ by the weak law of large numbers (WLLN), so it remains to upper bound the first term, henceforth denoted by $ \Prob{\event{A}}$, by a vanishing quantity as well. Note that
\begin{align}
    \Prob{\event{A}}
    &\leq \Prob{\log V(y^n|x^n(m)) \leq n(-D+\delta) \text{ for all } m \in [2:2^{nR}], y^n\in \typset{\epsilon}{n}(\pmf{\rv{Y}}) } \\
    &= \sum_{y^n \in \typset{\epsilon}{n}(\pmf{\rv{Y}})} \pmf{\rv{Y}^n}(y^n) \Prob{\log V(y^n|x^n(m)) \leq n(-D+\delta) \text{ for all } m \in [2:2^{nR}]} \\
    &= \sum_{y^n \in \typset{\epsilon}{n}(\pmf{\rv{Y}})} \pmf{\rv{Y}^n}(y^n) \left[ \sum_{x^n \colon \log V(y^n|x^n) \leq n(-D+\delta)}  \pmf{\rv{X}^n}(x^n) \right] ^{2^{nR}-1} \\
    &= \sum_{y^n \in \typset{\epsilon}{n}(\pmf{\rv{Y}})} \pmf{\rv{Y}^n}(y^n) \left[1- \sum_{x^n \colon \log V(y^n|x^n) > n(-D+\delta)}  \pmf{\rv{X}^n}(x^n) \right] ^{2^{nR}-1}.
\end{align}
Denoting $h(y^n) \triangleq \sum_{x^n \colon \log V(y^n|x^n) > n(-D+\delta)}  \pmf{\rv{X}^n}(x^n) $, and using the fact that $1-\alpha \leq e^{-\alpha}$ we obtain
\begin{align}
    \Prob{\event{A}}
    &\leq \sum_{y^n \in \typset{\epsilon}{n}(\pmf{\rv{Y}})} \pmf{\rv{Y}^n}(y^n) \exp \left( - h(y^n) \cdot 2^{nR} \right) \\
    &\leq \exp \left( - \min_{y^n \in \typset{\epsilon}{n}(\pmf{\rv{Y}})} h(y^n) \cdot 2^{nR} \right).
\end{align}
To complete the proof, we need to show that for every $y^n \in \typset{\epsilon}{n}(\pmf{\rv{Y}})$, $h(y^n)$ is exponentially no smaller than $2^{-n I'(\rv{X};\rv{Y})}$ when $\epsilon$ vanishes, and hence for every $R > I'(\rv{X};\rv{Y})$, $\Prob{\event{A}}$ is essentially less than $\exp\left(-e^{n(R-I'(\rv{X};\rv{Y}))} \right) \rightarrow 0$. To this end, let us further lower bound $h(y^n)$. First, note that for every $y^n \in \typset{\epsilon}{n}(\pmf{\rv{Y}})$,
\begin{align}
    h(y^n) 
    &= \sum_{x^n \colon \log V(y^n|x^n) > n(-D+\delta)}  \pmf{\rv{X}^n}(x^n) \\
    &= \sum_{ \set{T}(\pmf{\bv{x}|\bv{y}}) \colon \log V(\bv{y}|\bv{x}) \geq n(-D+\delta)} |\set{T}(\pmf{\bv{x}|\bv{y}})| \cdot 2^{-n[\kld{\pmf{\bv{x}}}{\pmf{\rv{X}}}+H(\pmf{\bv{x}})]} \\
    &\geq \max_{ \set{T}(\pmf{\bv{x}|\bv{y}}) \colon \log V(\bv{y}|\bv{x}) \geq n(-D+\delta)} |\set{T}(\pmf{\bv{x}|\bv{y}})| \cdot 2^{-n[\kld{\pmf{\bv{x}}}{\pmf{\rv{X}}}+H(\pmf{\bv{x}})]} .
\end{align}
Note that since $y^n$ is given, $\set{T}(\pmf{\bv{x}|\bv{y}})$ defines both $\pmf{\bv{x}}$ and $\pmf{\bv{x}|\bv{y}}$. Now, let
\begin{equation}
    \set{T} \triangleq \left\{ \bv{x} \colon \log V(\bv{y}|\bv{x}) > n(-D+\delta) \right\} \cap \typset{\epsilon}{n}(\pmf{\rv{X}}).
\end{equation}
Therefore
\begin{align}
    h(y^n) 
    &\geq \max_{\set{T}(\pmf{\bv{x}|\bv{y}}) \in \set{T}} |\set{T}(\pmf{\bv{x}|\bv{y}})| \cdot \pmf{\rv{X}^n}(\pmf{\bv{x})} \\
    &\geq \max_{\set{T}(\pmf{\bv{x}|\bv{y}})\in \set{T}} 2^{n[H(\pmf{\bv{x}|\bv{y}})-\delta(\epsilon)]} \cdot 2^{-n[H(\rv{X})+\epsilon']} \\
    &= 2^{-n [\min_{\pmf{\rv{X}|\rv{Y}} \in \set{T} } I(\pmf{\rv{X}}, \pmf{\rv{X} |\rv{Y}} ) + \epsilon' + \delta(\epsilon)]}.
\end{align}
This completed the proof of the converse.

==> sections/mmdec/mmdec_gaussian_channel.tex <==
Another example which might be rather interesting is the case where $\pmf{\rv{Y}|\rv{X}}$ is a classical Gaussian channel, that is:
\begin{equation}
    \rv{Y} = \rv{X} + \rv{N},
\end{equation}
where $\rv{N}$ is a complex normal signal, say take the notations from reference \cite{Caire2018}.
The decoder's mismatched metric is planned for:
\begin{equation}
    \rv{Y} = \rv{S} \rv{X} + \rv{N},
\end{equation}
where $\rv{S}$ now is not complex Gaussian as in \cite{Caire2018}, but an independent uniform phase distributed signal. That is it absolutely make the phase of $\rv{X}$ irrelevant. $\rv{S}$ is known to none. Evidently another interesting setting is that it is known to the relay, ala \cite{Caire2018} where the relay tries to convey that $\rv{S}$ with maximum accuracy to the final destination as well (over the common link where also $\rv{Y}$ is transferred).

Evidently for the mismatched decoder that assumes random phase ($\rv{S}$ known to none), it looks that one does not gain from the fact that the channel is the classical Gaussian channel ($\rv{Y} = \rv{X}+ \rv{N}$), and one can achieve the phase noise capacity (the optimal joint distribution of $\rv{X}$ is discrete with uncountable number of points), see \cite{Katz2004}.

==> sections/mmib_properties.tex <==
\subsection{Standard Information Bottleneck}
\input{sections/definitions/ib}

\subsection{Mismatched Information Bottleneck}
\input{sections/definitions/mmib}


==> sections/mmibdec_fading.tex <==
Let $I_{\mathsf{GMI}}(\pmf{\rv{X}}, \pmf{\rv{Z}|\rv{Y}} ,\lambda ) $ denote the dual objective function of the \acrshort{gmi} rate, i.e.,
\begin{equation}
    I_{\mathsf{GMI}}(f_{\rv{X} \rv{Z}} , \lambda ) 
    \triangleq  \int_{(x,z) \in \field{C}\times \field{C}} \mkern-55mu f(x,z) \log \frac{V(x,z)^{\lambda}}{\int_{x' \in \field{C}} f(x') V(x',z)^{\lambda} \mathrm{d}x'} \mathrm{d}x \mathrm{d}z.
\end{equation}
In particular, for the Gaussian setting, we have,
\begin{align}
    I_{\mathsf{GMI}}(f_{\rv{X} \rv{Z}} , \lambda ) 
    % &= \lambda \Exp{ \log V(\rv{X},\rv{Z})} - \Exp{ \log \Exp{ V(\bar{\rv{X}}, \rv{Z})^{\lambda}}} \\
    &= - \lambda \Exp{ |\rv{Z} - \hat{\rv{H}} \rv{X}|^2} - \Exp{ \log \Exp{ e^{- \lambda |\rv{Z}-\hat{\rv{H}} \rv{X} |^2} \big| \rv{Z} }}.
\end{align}
Implicit conditioning on $\hat{\rv{H}} = \hat{h}$ leads to:
\begin{multline}
    I_{\mathsf{GMI}}(f_{\rv{X} \rv{Z}} , \lambda ) = \log \left( 1+ \lambda |\hat{h}|^2 \Gamma \right) \\
    + \frac{\lambda \left[ \left( |\hat{h}|^2 
    + \Exp{|\Delta|^2|\hat{\rv{H}} = \hat{h}} \right) \Gamma +\sigma^2 + q \right]}{1+  \lambda |\hat{h}|^2 \Gamma } \\
    - \lambda \left(\Exp{|\Delta|^2|\hat{\rv{H}} = \hat{h}} \Gamma + \sigma^2 + q \right).
\end{multline}
This is a concave function of $\lambda$, with the maximum obtained when the derivative is zero, which is given by
\begin{equation}
    \lambda^* = \frac{1}{\Exp{|\Delta|^2|\hat{\rv{H}} = \hat{h}} \Gamma + \sigma^2 + q }.
\end{equation}
Substituting $\lambda^*$, we obtain
\begin{equation}
    I_{\mathsf{GMI}}(f_{\rv{X} \rv{Z}} , \lambda )  = \log \left( 1+ \frac{ |\hat{h}|^2 \Gamma}{\Exp{|\Delta|^2|\hat{\rv{H}} = \hat{h}} \Gamma + \sigma^2 + q } \right) .
\end{equation}
The proof is completed after averaging over $\hat{\rv{H}}$.

==> sections/mmrdib/lower_bound.tex <==
We use random coding. Let $\epsilon' < \epsilon$. Fix a \acrshort{pmf} $\pmf{\rv{X}}$. This induces a marginal \acrshort{pmf} for $\rv{Y}$, i.e., $\pmf{\rv{Y}}$.
\paragraph{Transmitter's Codebook Generation.}
 Randomly and independently generate $2^{nR}$ sequences $x^n(m)$, $m\in [1:2^{nR}]$, each according to $\pmf{\rv{X}^n} (x^n) = \prod_{i=1}^n \pmf{\rv{X}}(x_i)$. Those sequences constitute the transmitter's codebook. The codebook is revealed to the encoder and the decoder but not the relay.

\paragraph{Mismatched Relay's Codebook Generation.}
Given a conditional \acrshort{pmf} $\pmfQ{\rv{Z}|\rv{Y}}$, randomly and independently generate $2^{nB}$ sequences $z^n(w)$, $w \in [1:2^{nB}]$, each according to $ \pmfQ{\rv{Z}^n} (z^n) = \prod_{i=1}^n \pmfQ{\rv{Z}}(z_i)$, where $\pmfQ{\rv{Z}} = \pmfQ{\rv{Z}|\rv{Y}} \circ \pmf{\rv{Y}}$. These sequences constitute the relay's codebook. The codebook is revealed to the relay and the decoder but not to the transmitter.

\paragraph{Encoding.}
To send message $m \in [1:2^{nR}]$, transmitter sends $x^n(m)$.

\paragraph{Mismatched Relay Encoding.}
Upon observing $y^n$, the relay finds an index $w \in [1:2^{nB}]$  such that 
\begin{equation}
    \left( y^n,z^n(w) \right) \in \typset{\epsilon'}{n}(\pmfQ{\rv{Y}\rv{Z}}),
\end{equation}
where $\pmfQ{\rv{Y}\rv{Z}} = \pmfQ{\rv{Z}|\rv{Y}} \cdot \pmf{\rv{Y}}$.
If there is more than one such index, it select one of them uniformly at random. If there is no such index, it selects an index from $[1:2^{nB}]$ uniformly at random. The relay conveys the selected index $w$ to the decoder.

\paragraph{Mismatched Decoding.}
The receiver finds a unique message $\hat{m}$ such that
\begin{equation}
    \left(x^n(\hat{m}), z^n(w) \right) \in \typset{\epsilon, +}{n},
\end{equation}
where
\begin{equation}
    \typset{\epsilon. +}{n} \triangleq \left\{ (x^n,z^n) \colon \sum_{(a,c) \in \set{X} \times \set{Y}} \left[ \pmfQ{\rv{X}\rv{Z}}(a,c)- \pmf{\bv{x}\bv{z}} (a,c) \right] \mu_{ac} \leq \epsilon \right\},
\end{equation}
where $\pmfQ{\rv{X}\rv{Z}} = \pmfQ{\rv{Z}|\rv{Y}} \circ \pmf{\rv{X}\rv{Y}}$.
If there is none or more than one such message -- it declares an error event $\event{E}$.

\paragraph{Analysis of the probability of error at the mismatched relay.}
Let $\epsilon'' < \epsilon'$ and $\rv{W}$ denote the compression index chosen by the encoder at the relay. Since $\pmf{\rv{Y}^n}(y^n) = \prod_{i=1}^n \pmf{\rv{Y}}(y_i)$, then by the \acrshort{lln} 
\begin{equation}
    \lim_{n\rightarrow \infty} \Prob{\rv{Y}^n \in \typset{\epsilon''}{n}(\pmf{\rv{Y}})}  = 1.    
\end{equation}
Furthermore, $\rv{Z}^n(w)$, $w \in [1:2^{nB}]$, are random sequences independent of each other and $\rv{Y}^n$, distributed according to $\pmfQ{\rv{Z}^n(w)}(z^n) = \prod_{i=1}^n \pmfQ{\rv{Z}}(z_i)$. Thus, by the Covering Lemma \cite[Lemma 3.3]{gamal2011}, there exists $\delta(\epsilon')$ that tends to zero as $\epsilon' \rightarrow 0$ such that
\begin{equation}
    \lim_{n\rightarrow \infty} \Prob{\left( \rv{Y}^n, \rv{Z}^n(\rv{W}) \right) \notin \typset{\epsilon'}{n}(\pmfQ{\rv{Y}\rv{Z}})} =0,
\end{equation}
 if 
 \begin{equation}
     B > I(\pmf{\rv{Y}},\pmfQ{\rv{Z}|\rv{Y}}) + \delta(\epsilon').
 \end{equation}

\paragraph{Analysis of the probability of error at the mismatched decoder.}
Assume without loss of generality that $\rv{M} = 1$  is sent. The mismatched decoder makes an error \acrshort{iff} one or both of the following events occur:
\begin{align}
    \event{E}_1 &\triangleq \left\{ \left( \rv{X}^n(1), \rv{Z}^n(\rv{W}) \right) \notin \typset{\epsilon,+}{n}\right\}, \\
    \event{E}_2 &\triangleq \left\{ \left( \rv{X}^n(m), \rv{Z}^n(\rv{W}) \right) \in \typset{\epsilon,+}{n} \text{ for some } m \in [2:2^{nR}] \right\}.
\end{align}
Then by the union of events bound,
\begin{equation}
    \Prob{\event{E}} = \Prob{\event{E}_1 \cup \event{E}_2} \leq \Prob{\event{E}_1} + \Prob{\event{E}_2}.
\end{equation}
We bound each term. Consider the first term,
\begin{align}
    \Prob{\event{E}_1^c}
    &= \Prob{\left( \rv{X}^n(1), \rv{Z}^n(\rv{W}) \right) \in \typset{\epsilon,+}{n}} \\
    &\geq \Prob{\left( \rv{X}^n(1), \rv{Z}^n(\rv{W}) \right) \in \typset{\epsilon,+}{n},\left( \rv{X}^n(1),\rv{Y}^n, \rv{Z}^n(\rv{W}) \right) \in \typset{\epsilon}{n}(\pmfQ{\rv{X}\rv{Y}\rv{Z}})} \\
    &=  \Prob{\left( \rv{X}^n(1),\rv{Y}^n, \rv{Z}^n(\rv{W}) \right) \in \typset{\epsilon}{n}(\pmfQ{\rv{X}\rv{Y}\rv{Z}})} \cdot  \Prob{\left( \rv{X}^n(1), \rv{Z}^n(\rv{W}) \right) \in \typset{\epsilon,+}{n}| \left( \rv{X}^n(1),\rv{Y}^n, \rv{Z}^n(\rv{W}) \right) \in \typset{\epsilon}{n}(\pmfQ{\rv{X}\rv{Y}\rv{Z}})}.
\end{align}
Consider the complement of the first multiplicand,
\begin{align}
    &\Prob{\left( \rv{X}^n(1),\rv{Y}^n, \rv{Z}^n(\rv{W}) \right) \notin \typset{\epsilon}{n}(\pmfQ{\rv{X}\rv{Y}\rv{Z}})} \\
    &= \Prob{ \left\{ \left( \rv{X}^n(1),\rv{Y}^n \right) \notin \typset{\epsilon}{n}(\pmf{\rv{X}\rv{Y}}) \right\} \cup \left\{ \left\{ \left( \rv{X}^n(1),\rv{Y}^n, \rv{Z}^n(\rv{W}) \right) \notin \typset{\epsilon}{n}(\pmfQ{\rv{X}\rv{Y}\rv{Z}}) \right\} \cap \left\{ \left( \rv{X}^n(1),\rv{Y}^n \right) \in \typset{\epsilon}{n}(\pmf{\rv{X}\rv{Y}}) \right\} \right\} } \\
    &\leq \Prob{ \left\{ \left( \rv{X}^n(1),\rv{Y}^n \right) \notin \typset{\epsilon}{n}(\pmf{\rv{X}\rv{Y}}) \right\} } + \Prob{ \left\{ \left( \rv{X}^n(1),\rv{Y}^n, \rv{Z}^n(\rv{W}) \right) \notin \typset{\epsilon}{n}(\pmfQ{\rv{X}\rv{Y}\rv{Z}}) \right\} \cap \left\{ \left( \rv{X}^n(1),\rv{Y}^n \right) \in \typset{\epsilon}{n}(\pmf{\rv{X}\rv{Y}}) \right\}  } 
\end{align}
Since $\pmf{\rv{X}^n(1)\rv{Y}^n}(x^n,y^n) = \prod_{i=1}^n \pmf{\rv{X}\rv{Y}} (x_i,y_i)$ then by the \acrshort{lln} the first term tends to zero as $n\rightarrow \infty$. Furthermore, since $\left( \rv{X}^n(1),\rv{Y}^n \right) \in \typset{\epsilon}{n}(\pmf{\rv{X}\rv{Y}})$ and $\rv{Z}^n (\rv{W})\sim \pmfQ{\rv{Z}^n|\rv{Y}^n}$, by Markov Lemma \cite[Lemma 12.1]{gamal2011}, the second term also goes to zero as $n\rightarrow \infty$.

To this end, we have shown that $\Prob{\left( \rv{X}^n(1),\rv{Y}^n, \rv{Z}^n(\rv{W}) \right) \in \typset{\epsilon}{n}(\pmfQ{\rv{X}\rv{Y}\rv{Z}})} $ tends to 1 as $n \rightarrow \infty$.
Note that for every $x^n \in \typset{\epsilon''}{n}(\pmf{\rv{x}})$, $y^n \in \typset{\epsilon'}{n}(\pmf{\rv{Y}|\rv{X}}) $ and $z^n \in \typset{\epsilon}{(n)}(\pmfQ{\rv{Z}|\rv{Y}})$ we have
\begin{align}
    \pmf{\bv{x} \bv{y} \bv{z}} (a,b,c)
    &= \frac{\sum_{i=1}^n \indicator{x_i=a,y_i=b,z_i=c}}{n} \\
    &= \frac{\sum_{i=1}^n \indicator{x_i=a}}{n} \frac{\sum_{i=1}^n \indicator{x_i=a,y_i=b,z_i=c}}{\sum_{i=1}^n \indicator{x_i=a}} \\
    &= \pmf{\bv{x}}(a) \frac{\sum_{i=1}^n \indicator{x_i=a,y_i=b}}{\sum_{i=1}^n \indicator{x_i=a}} \frac{\sum_{i=1}^n \indicator{x_i=a,y_i=b,z_i=c}}{\sum_{i=1}^n \indicator{x_i=a,y_i=b}} \\
    &\geq \pmf{\rv{X}}(a) (1-\epsilon'') \cdot \pmf{\rv{Y}|\rv{X}} (b|a) (1-\epsilon') \cdot \pmfQ{\rv{Z}|\rv{Y}} (c|b) (1-\epsilon) \\
    &= \pmfQ{\rv{X}\rv{Y}\rv{Z}}(a,b,c) (1-\epsilon'')(1-\epsilon')(1-\epsilon).
\end{align}
This implies that
\begin{align}
    \sum_{(a,c) \in \set{X}\times\set{Z}} \left[\pmfQ{\rv{X}\rv{Z}}(a,c) - \pmf{\bv{x}(1) \bv{z}(W)}(a,c)  \right] \mu_{ac}
    &\leq  \left(1-(1-\epsilon'')(1-\epsilon')(1-\epsilon) \right) \sum_{(a,c) \in \set{X} \times \set{Z}} \mu_{ac} \\
    &= (\epsilon''+\epsilon'+\epsilon) \sum_{(a,c) \in \set{X} \times \set{Z}} \mu_{ac} \leq \epsilon_+.
\end{align}
Therefore, $\Prob{\event{E}_1}$ tends to zero as $n$ tends to infinity.
Consider the second term. Using the fact that for every $m \neq 1$ and $W$ the pair $(\rv{X}^n(m),\rv{Z}^n(W))$ distributed according to $\pmf{\rv{X}^n(m)\rv{Z}^n(W)}(x^n,z^n) = \prod_{i=1}^n \pmf{\rv{X}} (x_i) \pmf{\rv{Z}} (z_i)$, utilizing Sanov's theorem we obtain the following bound
\begin{align}
    \Prob{\event{E}_2}
    &= \Prob{\left( \rv{X}^n(m), \rv{Z}^n(W) \right) \in \typset{\epsilon,+}{n} \text{ for some } m \in [2:2^{nR}]} \\
    &\leq \sum_{m=2}^{2^{nR}} \Prob{\left( \rv{X}^n(m), \rv{Z}^n(W) \right) \in \typset{\epsilon,+}{n} } \\
    &\leq \sum_{m=2}^{2^{nR}} (n+1)^{|\set{X}|\cdot |\set{Z}| } 2^{-n\kld{\pmf{}^*}{\pmf{\rv{X}}\pmfQ{Z}} }\\
    &\leq (n+1)^{|\set{X}|\cdot |\set{Z}| } 2^{n(R-\kld{\pmf{}^*}{\pmf{\rv{X}}\pmfQ{Z}}) },
\end{align}
where
\begin{equation}
    \pmf{}^* = \argmin_{\pmf{} \in \typset{\epsilon, + }{n}} \kld{\pmf{}}{\pmf{\rv{X}} \pmfQ{\rv{Z}}}.
\end{equation}
Thus $\Prob{\event{E}_2}$ tends to zero as $ n \rightarrow \infty $ if $R < \kld{\pmf{}^*}{\pmf{\rv{X}}\pmfQ{\rv{Z}}})  - \delta(\epsilon) $.

==> sections/mmrdib_main_results.tex <==
\begin{figure}[b]
    \centering
    \input{./figures/mmrdib/block_diagram}
    \caption{Oblivious Communication System with Mismatched Relay and Mismatched Decoder}
    \label{fig:mmrdib_communication_diagram}
\end{figure}

Consider the 3-node point-to-point communication system with a relay depicted in \autoref{fig:mmrdib_communication_diagram}. The sender wishes to communicate a message $\rv{M}$ to the receiver with the help of the relay. We consider the \acrfull{dmmmrdibc} model $(\rv{X}, \pmf{\rv{Y}|\rv{X}},  \set{Y}, \set{Z},V(z|x))$ that consists of two finite sets $\set{X}$, $\set{Y}$, and a collection of conditional \acrshort{pmf}s $\pmf{\rv{Y}|\rv{X}}$ on $\set{Y}$ and $V(z|x)$  on $\set{Z}$.

A $(2^{nR},2^{nB},n)$ code for the \acrshort{dmmmrdibc} consists of
\begin{itemize}
    \item a message set $\set{M} = [1:2^{nR}]$,
    % \item a representation set $\set{W} = [1:2^{nB}]$,
    \item an encoder that assigns a codeword $x^n(m)$ to each message $m \in \set{M}$,
    \item a mismatched relay encoder that assigns an index $w \in \set{W}$ to each received sequence $y^n \in \set{Y}^n$ using a random coding according to some fixed $\pmfQ{\rv{Z}|\rv{Y}}$, and
    \item a mismatched decoder that assigns an estimate $\hat{m}$ or an error message e to each received representation index $w \in \set{W}$ according to a mismatched metric
    \begin{equation}
        \hat{m}(z^n) = \argmax_{m \in \set{M}} \pmfQ{\rv{Z}|\rv{X}}^{(n)}(z^n|x^n(m)) = \argmax_{m \in \set{M}} \prod_{i=1}^n \pmfQ{\rv{Z}|\rv{X}} (z_i|x_i(m)).
    \end{equation}
\end{itemize}
We denote
\begin{equation}
    \sum_{x \in \set{X}} \sum_{y \in \set{Y}} \sum_{z \in \set{Z}}  \pmf{\rv{X}}(x) \pmf{\rv{Y}|\rv{X}} (y|x) \pmf{\rv{Z}|\rv{Y}}(z|y) \log  V(z|x) = -D .
\end{equation}
We assume that the message $\rv{M}$ is uniformly distributed over the message set. The average probability of error is defined as $P_e^{(n)} = \Prob{\hat{\rv{M}} \neq \rv{M}}$. A rate $R$ is said to be \textit{achievable} for the \acrshort{dmmmribc} is there exists a sequence of $(2^{nR},2^{nB},n)$ codes such that $\lim_{n\rightarrow \infty} P_e^{(n)} = 0$. The \textit{capacity} $C$ of the \acrshort{dmmmribc} is the supremum of all achievable rates. 

Our main result is stated in the following theorem.
\begin{theorem} \label{theorem:mmrdib_rate}
    The random coding capacity of the oblivious mismatched relay channel with mismatched decoder is given by:
    \begin{equation}
        \begin{aligned}
            &C(\pmfQ{\rv{Z}|\rv{Y}}, \pmfQ{\rv{Z}|\rv{X}}) =
            && \max_{\pmf{\rv{X}}} 
            &&\min_{\pmfQ{\rv{Y}|\rv{X}}}
            && I(\pmf{\rv{X}}, \pmf{\rv{Z}|\rv{Y}} \circ \pmfQ{\rv{Y}|\rv{X}}) \\
            &&&&& \text{subject to} 
            && \sum_{x\in \set{X}} \pmf{\rv{X}}(x) \pmfQ{\rv{Y}|\rv{X}}(y|x) = \pmf{\rv{Y}} (y) \\
            &&&&&&& \sum_{x \in \set{X}} \sum_{y \in \set{Y}} \sum_{z \in \set{Z}} \pmf{\rv{X}}(x) \pmfQ{\rv{Y}|\rv{X}} (y|x) \pmfQ{\rv{Z}|\rv{Y}} (z|y) \log V(z|x) \geq -D.
        \end{aligned}
    \end{equation}
    if $I(\pmf{\rv{Y}}^*,\pmfQ{\rv{Z}|\rv{Y}}) < B $ and zero otherwise.
\end{theorem}
\begin{proof}
    The proof of the direct part is in App. \ref{appendix:theorem_mmrdib_rate_direct_proof}.
    % and App. \ref{appendix:theorem_mmrdib_rate_converse_proof}, respectively.
\end{proof}



==> sections/mmrscll_main_results.tex <==
\begin{figure}[b]
    \centering
    \input{./figures/mmrscll/block_diagram}
    \caption{Mismatched Remote Source Coding block daigram}
    \label{fig:mmrscll_block_diagram}
\end{figure}

Consider the remote source coding diagram with mismatched encoder illustrated in \autoref{fig:mmrscll_block_diagram}.


Let $\{\rv{X}_i,\rv{Y}_i \}_{i=1}^n = (\rv{X}^n,\rv{Y}^n)$ be a sequence of $n$ \acrfull{iid} random variables distributed according to the joint \acrshort{pmf} $\pmf{\rv{X}\rv{Y}} = \pmf{\rv{X}} \pmf{\rv{Y}|\rv{X}}$.

In this section, we consider the reproduction alphabet $\set{Z}$ to be equal to the set of probability distributions over the source alphabet $\set{X}$. For a vector $\rv{Z}^n \in \set{Z}^n$, we will use the notation $\rv{Z}_i$ to mean the $i^{th}$ coordinate of $\rv{Z}^n$ (which is a probability distribution on $\set{X}$), and $\rv{Z}_i(x)$ is the probability outcome $x \in \set{X}$.

A $(2^{nR}, D,n)$ rate-distortion code consists of
\begin{itemize}
    \item an index set $\set{W} = [1:2^{nR}]$,
    \item an encoder that assigns an index $w \in \set{W}$ to each received sequence $ y^n \in \set{Y}^n$, and
    \item a decoder that assigns an estimate $z^n $ to each received representation $w \in \set{W}$.
\end{itemize}
The set $\set{C} = \{z^n(1),z^n(2),\dots,z^n(|\set{W}|) \}$ constitutes the codebook.

The expected distortion associated with $(2^{nR},n)$ lossy source code is defined as
\begin{equation}
    \Exp{d(\rv{X}^n,\rv{Z}^n)} = \sum_{x^n \in \set{X}^n} \pmf{\rv{X}^n}(x^n) d(x^n,z^n).
\end{equation}
We restrict here the fidelity measure to log-loss, i.e.,
\begin{equation}
    d(x,z) = \log \frac{1}{z(x)}
\end{equation}
where $z(x)$ is the $x$th coordinate of the probability vector $z$.
A rate distortion pair $(R,D)$ is said to be achievable for the DM-IB if there exists a blocklength $n$, encoding function $f^{(n)}$ and a decoder $g^{(n)}$  such that  $D \geq \Exp{d(\rv{X}^n,\rv{Z}^n)}$, where
\begin{equation}
    \rv{Z}^n = g^{(n)}(f^{(n)}(\rv{Y}^n)).
\end{equation}
The rate-distortion function $R(D)$ is the infimum of rated such that $(R,D)$ is achievable.

\begin{theorem}
    The remote rate-distortion function for a \acrshort{dms} $ \pmf{\rv{X}\rv{Y}}$ and a log-loss distortion measure $d(x,z) = -\log z(x)$ is
    \begin{equation}
        \begin{aligned}
            &R(D) =
            && \min_{\pmf{\rv{Z}|\rv{Y}}} 
            && I(\rv{Y};\rv{Z}) \\
            &&& \text{subject to}
            && H(\rv{X}|\rv{Z}) \geq D.
        \end{aligned}
    \end{equation}
    where $|\set{Z}| \leq |\set{Y}|+1$.
\end{theorem}

\subsection{Proof of Converse}
\input{sections/source_coding/converse_proof}


\subsection{Proof of Achievability}
\paragraph{Codebook generation.} For every $\epsilon_d>0$, fix the conditional \acrshort{pmf} $\pmf{\rv{Z}|\rv{Y}}$ that induces $\Exp{d(\rv{X},\rv{Z})} \leq D/(1+\epsilon_d)$. Randomly and independently generate $2^{nR}$ sequences $z^n(w)$, $w \in [1:2^{nR}]$, each according to $\prod_{i=1}^n \pmf{\rv{Z}}(z_i)$. These sequences constitute the source-coding codebook $\set{C}$, which is revealed to the encoder and the decoder.

\paragraph{Encoding.} Upon observing $y^n$, the encoder finds an index $w$ such that $(y^n,z^n(w)) \in \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}})$. If there is more than one such index, it selects one of them uniformly at random. If there is no such index, it select an index from $[1:2^{nR}]$ uniformly at random. The encoder sends the index $w$ to the decoder.

\paragraph{Decoding}
Upon receiving the index $w$, the decoder sets the reconstruction sequence $z^n = z^n(w)$.

\paragraph{Analysis of expected distortion.}
Let $\epsilon' < \epsilon$ and $\rv{W}$ be the index chosen by the encoder, We bound the distortion averaged over the random choice of the codebook $\set{C}$. Define the ``encoding error" event
\begin{equation}
    \set{E} = \{ (\rv{Y}^n,\rv{Z}^n(\rv{W})) \notin \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}}) \},
\end{equation}
and consider the events
\begin{align}
    \set{E}_1 &= \{ \rv{Y}^n \notin \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}}) \},\\
    \set{E}_2 &= \{ \rv{Y}^n \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}}), (\rv{Y}^n,\rv{Z}^n(w)) \notin \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}}) \text{ for all } w\in [1:2^{nR}] \}.
\end{align}
Then by the union of events bound,
\begin{equation}
    \Prob{\event{E}} = \Prob{\event{E}_1 \cup \event{E}_2} \leq \Prob{\event{E}_1} + \Prob{\event{E}_2}.
\end{equation}
We bound each term. Since $\pmf{\rv{Y}^n} (y^n) = \prod_{i=1}^n \pmf{\rv{Y}}(y_i) $, by the \acrfull{lln}, the first term $\Prob{\event{E}_1}$ tends to zero as $n \rightarrow \infty $. Consider the second term
\begin{align}
    \Prob{\event{E}_2}
    &= \Prob{\rv{Y}^n \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}}), (\rv{Y}^n,\rv{Z}^n(w)) \notin \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}}) \text{ for all } w\in [1:2^{nR}]} \\
    %&= \sum_{y^n \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}})} \Prob{(\rv{Y}^n,\rv{Z}^n(w)) \notin \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}}) \text{ for all } w\in [1:2^{nR}] \bigg| \rv{Y}^n=y^n} \pmf{\rv{Y}^n}(y^n) \\
    &= \sum_{y^n \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}})} \Prob{(y^n,\rv{Z}^n(w)) \notin \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}}) \text{ for all } w\in [1:2^{nR}] \bigg| \rv{Y}^n=y^n} \pmf{\rv{Y}^n}(y^n) \\
    &= \sum_{y^n \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}})} \prod_{w=1}^{2^{nR}} \Prob{(y^n,\rv{Z}^n(w)) \notin \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}}) } \pmf{\rv{Y}^n}(y^n) \\
    &= \sum_{y^n \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}})} \left( \Prob{(y^n,\rv{Z}^n(1)) \notin \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}}) } \right)^{2^{nR}} \pmf{\rv{Y}^n}(y^n).
\end{align}
Since $y^n \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}})$ and $\rv{Z}^n(1) \sim \prod_{i=1}^n \pmf{\rv{Z}} (z_i)$ it follows by the joint typicality lemma \cite[Ch. 2.5]{gamal2011} that for $n$ sufficiently large
\begin{equation}
    \Prob{(y^n,\rv{Z}^n(1)) \in \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}}) }  \geq 2^{-n(I(\rv{Y};\rv{Z}) + \delta(\epsilon))},
\end{equation}
where $\delta(\epsilon)$ tends to zero as $\epsilon \rightarrow 0$. Since $(1-x)^k \leq e^{-kx}$ for $x \in [0,1]$ and $k>0$, we have
\begin{align}
    \sum_{y^n \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}})} \left( \Prob{(y^n,\rv{Z}^n(1)) \notin \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}}) } \right)^{2^{nR}}
    & \leq  \left(1 - 2^{-n(I(\rv{Y};\rv{Z}) + \delta(\epsilon))} \right)^{2^{nR}} \\
    & \leq  e^{-2^{-n(I(\rv{Y};\rv{Z})-R + \delta(\epsilon))}}
\end{align}
which tends to zero as $n \rightarrow \infty$ if $R > I(\rv{Y};\rv{Z}) + \delta(\epsilon)$.

Define the ``typical distortion error" event
\begin{equation}
    \set{E}_d = \{ (\rv{X}^n, \rv{Y}^n, \rv{Z}^n(\rv{W})) \notin \set{T}_{\epsilon_d}^{(n)}(\pmf{\rv{X} \rv{Y}\rv{Z}}) \} \cap \event{E}^c.
\end{equation}
By Markov lemma \cite[Lemma 12.1]{gamal2011}, $\lim_{n\rightarrow \infty} \Prob{\event{E}_d} = 0$.
Now, by the law of total expectation and the typical average lemma,
\begin{align}
    \Exp[\set{C},\rv{X}^n]{d(\rv{X}^n,\rv{Z}^n(\rv{W}))}
    &= \Prob{\event{E}_d} \Exp[\set{C},\rv{X}^n]{d(\rv{X}^n,\rv{Z}^n(\rv{W})) | \event{E}_d} + \Prob{\event{E}_d^c} \Exp[\set{C},\rv{X}^n]{d(\rv{X}^n,\rv{Z}^n(\rv{W})) | \event{E}_d^c} \\
    &\leq \Prob{\event{E}_d} d_{\max}  + \Prob{\event{E}^c} \Exp[\set{C},\rv{X}^n]{d(\rv{X}^n,\rv{Z}^n(\rv{W})) | \event{E}_d^c}
\end{align}
where $d_{\max} = \max_{(x,z)\in \set{X} \times \set{Z}} d(x,z)$.
Note that
\begin{equation}
    \Exp[\set{C},\rv{X}^n]{d(\rv{X}^n,\rv{Z}^n(\rv{W})) | \event{E}_d^c}
    = \sum_{(x^n,z^n) \in \typset{\epsilon}{n}(\pmf{\rv{X}\rv{Z}})} \pmf{\rv{X}^n \rv{Z}^n}(x^n,z^n) d(x^n,z^n).
\end{equation}
For every $(x^n,z^n) \in \typset{\epsilon_d}{n}(\pmf{\rv{X}\rv{Z}})$ we have
\begin{align}
    d(x^n,z^n)
    &= \frac{1}{n} \sum_{i=1}^n d(x_i,z_i) \\
    &= \sum_{(a,c) \in \set{X} \times \set{Z}} \pmf{\bv{x} \bv{z}}(a,c) d(a,c) \\
    &\leq (1+\epsilon_d) \sum_{(a,c) \in \set{X} \times \set{Z}} \pmf{\rv{X}\rv{Z}} (a,c) d(a,c) \\
    &= (1+\epsilon_d) \Exp{d(\rv{X},\rv{Z})} \leq  D.
\end{align}
Thus,
\begin{equation}
    \Exp[\set{C},\rv{X}^n]{d(\rv{X}^n,\rv{Z}^n(\rv{W})) | \event{E}_d^c} \leq D
\end{equation}
and
\begin{equation}
    \limsup_{n \rightarrow \infty} \Exp[\set{C},\rv{X}^n]{d(\rv{X}^n,\rv{Z}^n(\rv{W}))} \leq D.
\end{equation}


==> sections/research_questions.tex <==
In this section we gather the possible research questions we would like to address in this work.
\begin{enumerate}
    \item Evaluation of the MMIB for the Gaussian and binary $(\rv{X},\rv{Y})$.
\end{enumerate}

==> sections/source_coding/converse_proof.tex <==
Consider the system diagram illustrated in \autoref{fig:ib_source_coding_diagram}.

For some arbitrary $w \in \set{W}$ denote $\Tilde{z}^n = g^{(n)}(w)$. Since $ \{ \Tilde{z}_i (x) \}_{x \in \set{X}}$ is a probability vector , then $s(x^n|w) \triangleq \prod_{i=1}^n \Tilde{z}(x_i) $ is also a probability vector, i.e. gives a probability to every  $x^n \in \set{X}^n$. Consider the conditional expected distortion as follows
\begin{align}
    \Exp{d(\rv{X}^n,\rv{Z}^n)|\rv{W}=w}
    &= \sum_{(x^n, z^n) \in \set{X}^n \times \set{Z}^n} \pmf{\rv{X}^n \rv{Z}^n|\rv{W}}(x^n,z^n|w)d(x^n,z^n) \\
    &= \sum_{(x^n, z^n) \in \set{X}^n \times \set{Z}^n} \pmf{\rv{X}^n|\rv{W}}(x^n|w) \pmf{\rv{Z}^n|\rv{W} \rv{X}^n}(z^n|w,x^n) d(x^n,z^n) \\
    &= \sum_{(x^n, z^n) \in \set{X}^n \times \set{Z}^n} \pmf{\rv{X}^n|\rv{W}}(x^n|w) \pmf{\rv{Z}^n|\rv{W}} (z^n|w) d(x^n,z^n) \\
    &= \sum_{(x^n, z^n) \in \set{X}^n \times \set{Z}^n} \pmf{\rv{X}^n|\rv{W}}(x^n|w) 
    \indicator{z^n = g^{(n)} (w)} d(x^n,z^n) \\
    &= \sum_{x^n \in \set{X}^n} \pmf{\rv{X}^n|\rv{W}}(x^n|w) 
     d(x^n,g^{(n)}(w)) \\
    &= \sum_{x^n \in \set{X}^n} \pmf{\rv{X}^n|\rv{W}}(x^n|w) 
     d(x^n,\Tilde{z}^n) \\
    &= \frac{1}{n} \sum_{i=1}^n \sum_{x^n \in \set{X}^n} \pmf{\rv{X}^n|\rv{W}}(x^n|w) \log \frac{1}{\Tilde{z}_i(x_i)} \\
    &= \frac{1}{n}  \sum_{x^n \in \set{X}^n} \pmf{\rv{X}^n|\rv{W}}(x^n|w) \sum_{i=1}^n \log \frac{1}{\Tilde{z}_i(x_i)} \\
    &= \frac{1}{n}  \sum_{x^n \in \set{X}^n} \pmf{\rv{X}^n|\rv{W}}(x^n|w) \log \frac{1}{\prod_{i=1}^n \tilde{z}_i(x_i)} \\
    &= \frac{1}{n}  \sum_{x^n \in \set{X}^n} \pmf{\rv{X}^n|\rv{W}}(x^n|w) \log \frac{\pmf{\rv{X}^n|\rv{W}}(x^n|w)}{s(x^n|w)} + H(\rv{X}^n|\rv{W}=w) \\
    &= \frac{1}{n} D( \pmf{\rv{X}^n|\rv{W}=w} \|  s(\rv{X}^n|w) ) + \frac{1}{n}  H(\rv{X}^n|\rv{W}=w) \\
    &\geq \frac{1}{n} H(\rv{X}^n|\rv{W}=w).
\end{align}
Taking the expectation over all values of $\rv{W}$ we obtain the following result:
\begin{equation}
    D \geq \Exp{d(\rv{X}^n,\rv{Z}^n)} \geq \frac{1}{n} H(\rv{X}^n|\rv{W}).
\end{equation}
Next we develop a lower bound for the achievable rate. We denote $\rv{Z}_i \triangleq (\rv{W},\rv{Y}^{i-1}) $. With this notation established, we have the following string
of inequalities:

\begin{align}
    nR
    &\geq H(\rv{W}) \\
    &\geq I(\rv{W};\rv{Y}^n) \\
    &= I(\rv{W};\rv{X}^n,\rv{Y}^n) \\
    &= I(\rv{W};\rv{X}^n) + I(\rv{W};\rv{Y}^n|\rv{X}^n) \\
    &= H(\rv{X}^n) - H(\rv{X}^n|\rv{W}) + \sum_{i=1}^n I(\rv{Y}_i;\rv{W}|\rv{X}^n,\rv{Y}^{i-1}) \\
    &\geq  n H(\rv{X}) + \sum_{i=1}^n H(\rv{Y}_i|\rv{X}^n,\rv{Y}^{i-1}) - H(\rv{Y}_i|\rv{W},\rv{X}^n,\rv{Y}^{i-1}) - nD \\
    &\geq n H(\rv{X}) + \sum_{i=1}^n H(\rv{Y}_i|\rv{X}_i) - H(\rv{Y}_i|\rv{W},\rv{X}_i,\rv{Y}^{i-1}) - nD \\
    &= n H(\rv{X}) + nH(\rv{Y}|\rv{X}) -\sum_{i=1}^n  H(\rv{Y}_i|\rv{Z}_i,\rv{X}_i) - nD \\ 
    &= n H(\rv{X}) + nH(\rv{Y}|\rv{X}) - n H(\rv{Y}_\rv{Q}|\rv{X}_{\rv{Q}},\rv{Z}_{\rv{Q}},\rv{Q})  - nD \\
    &= n H(\rv{X}) + nH(\rv{Y}|\rv{X}) - n H(\rv{Y}|\rv{X},\rv{Z})  - nD \\
    &= n H(\rv{X}) + n I(\rv{Y};\rv{Z}|\rv{X})  - nD \\
\end{align}

Similarly,
\begin{align}
    H(\rv{X}^n|\rv{W})
    &= \sum_{i=1}^n H(\rv{X}_i|\rv{W}, \rv{X}^{i-1}) \\
    &\geq \sum_{i=1}^n H(\rv{X}_i|\rv{W}, \rv{X}^{i-1}, \rv{Y}^{i-1} ) \\
    &= \sum_{i=1}^n H(\rv{X}_i|\rv{W}, \rv{Y}^{i-1} ) \\
    &= \sum_{i=1}^n H(\rv{X}_i|\rv{Z}_i ) \\
    &= n H(\rv{X}_{\rv{Q}}|\rv{Z}_{\rv{Q}},\rv{Q}) \\
    &= n H(\rv{X}|\rv{Z}).
\end{align}
We conclude that if $(R,D)$ is strict-sense achievable for the remote source coding with log-loss problem, then
\begin{align}
    R &\geq H(\rv{X}) + I(\rv{Y};\rv{Z}|\rv{X})  - D \\
    D & \geq H(\rv{X}|\rv{Z}),
\end{align}
for some joint distribution of the form
\begin{equation}
    \pmf{\rv{X}\rv{Y}} \pmf{\rv{Z}|\rv{Y}}.
\end{equation}


==> sections/source_coding_problem_formulation.tex <==
\begin{figure}[b]
    \centering
    \input{./figures/ib/source_coding_diagram}
    \caption{Remote Source Coding}
    \label{fig:ib_source_coding_diagram}
\end{figure}

Consider the remote source coding diagram illustrated in \autoref{fig:ib_source_coding_diagram}.


Let $\{\rv{X}_i,\rv{Y}_i \}_{i=1}^n = (\rv{X}^n,\rv{Y}^n)$ be a sequence of $n$ \acrfull{iid} random variables distributed according to the joint \acrshort{pmf} $\pmf{\rv{X}\rv{Y}} = \pmf{\rv{X}} \pmf{\rv{Y}|\rv{X}}$.

In this section, we consider the reproduction alphabet $\set{Z}$ to be equal to the set of probability distributions over the source alphabet $\set{X}$. For a vector $\rv{Z}^n \in \set{Z}^n$, we will use the notation $\rv{Z}_i$ to mean the $i^{th}$ coordinate of $\rv{Z}^n$ (which is a probability distribution on $\set{X}$), and $\rv{Z}_i(x)$ is the probability outcome $x \in \set{X}$.

A $(2^{nR}, D,n)$ rate-distortion code consists of
\begin{itemize}
    \item an index set $\set{W} = [1:2^{nR}]$,
    \item an encoder that assigns an index $w \in \set{W}$ to each received sequence $ y^n \in \set{Y}^n$, and
    \item a decoder that assigns an estimate $z^n $ to each received representation $w \in \set{W}$.
\end{itemize}
The set $\set{C} = \{z^n(1),z^n(2),\dots,z^n(|\set{W}|) \}$ constitutes the codebook.

The expected distortion associated with $(2^{nR},n)$ lossy source code is defined as
\begin{equation}
    \Exp{d(\rv{X}^n,\rv{Z}^n)} = \sum_{x^n \in \set{X}^n} \pmf{\rv{X}^n}(x^n) d(x^n,z^n).
\end{equation}
We restrict here the fidelity measure to log-loss, i.e.,
\begin{equation}
    d(x,z) = \log \frac{1}{z(x)}
\end{equation}
where $z(x)$ is the $x$th coordinate of the probability vector $z$.
A rate distortion pair $(R,D)$ is said to be achievable for the DM-IB if there exists a blocklength $n$, encoding function $f^{(n)}$ and a decoder $g^{(n)}$  such that  $D \geq \Exp{d(\rv{X}^n,\rv{Z}^n)}$, where
\begin{equation}
    \rv{Z}^n = g^{(n)}(f^{(n)}(\rv{Y}^n)).
\end{equation}
The rate-distortion function $R(D)$ is the infimum of rated such that $(R,D)$ is achievable.

\begin{theorem}
    The remote rate-distortion function for a \acrshort{dms} $ \pmf{\rv{X}\rv{Y}}$ and a log-loss distortion measure $d(x,z) = -\log z(x)$ is
    \begin{equation}
        \begin{aligned}
            &R(D) =
            && \min_{\pmf{\rv{Z}|\rv{Y}}} 
            && I(\rv{Y};\rv{Z}) \\
            &&& \text{subject to}
            && H(\rv{X}|\rv{Z}) \geq D.
        \end{aligned}
    \end{equation}
    where $|\set{Z}| \leq |\set{Y}|+1$.
\end{theorem}

\subsection{Proof of Converse}
\input{sections/source_coding/converse_proof}


\subsection{Proof of Achievability}
\paragraph{Codebook generation.} For every $\epsilon_d>0$, fix the conditional \acrshort{pmf} $\pmf{\rv{Z}|\rv{Y}}$ that induces $\Exp{d(\rv{X},\rv{Z})} \leq D/(1+\epsilon_d)$. Randomly and independently generate $2^{nR}$ sequences $z^n(w)$, $w \in [1:2^{nR}]$, each according to $\prod_{i=1}^n \pmf{\rv{Z}}(z_i)$. These sequences constitute the source-coding codebook $\set{C}$, which is revealed to the encoder and the decoder.

\paragraph{Encoding.} Upon observing $y^n$, the encoder finds an index $w$ such that $(y^n,z^n(w)) \in \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}})$. If there is more than one such index, it selects one of them uniformly at random. If there is no such index, it select an index from $[1:2^{nR}]$ uniformly at random. The encoder sends the index $w$ to the decoder.

\paragraph{Decoding}
Upon receiving the index $w$, the decoder sets the reconstruction sequence $z^n = z^n(w)$.

\paragraph{Analysis of expected distortion.}
Let $\epsilon' < \epsilon$ and $\rv{W}$ be the index chosen by the encoder, We bound the distortion averaged over the random choice of the codebook $\set{C}$. Define the ``encoding error" event
\begin{equation}
    \set{E} = \{ (\rv{Y}^n,\rv{Z}^n(\rv{W})) \notin \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}}) \},
\end{equation}
and consider the events
\begin{align}
    \set{E}_1 &= \{ \rv{Y}^n \notin \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}}) \},\\
    \set{E}_2 &= \{ \rv{Y}^n \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}}), (\rv{Y}^n,\rv{Z}^n(w)) \notin \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}}) \text{ for all } w\in [1:2^{nR}] \}.
\end{align}
Then by the union of events bound,
\begin{equation}
    \Prob{\event{E}} = \Prob{\event{E}_1 \cup \event{E}_2} \leq \Prob{\event{E}_1} + \Prob{\event{E}_2}.
\end{equation}
We bound each term. Since $\pmf{\rv{Y}^n} (y^n) = \prod_{i=1}^n \pmf{\rv{Y}}(y_i) $, by the \acrfull{lln}, the first term $\Prob{\event{E}_1}$ tends to zero as $n \rightarrow \infty $. Consider the second term
\begin{align}
    \Prob{\event{E}_2}
    &= \Prob{\rv{Y}^n \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}}), (\rv{Y}^n,\rv{Z}^n(w)) \notin \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}}) \text{ for all } w\in [1:2^{nR}]} \\
    %&= \sum_{y^n \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}})} \Prob{(\rv{Y}^n,\rv{Z}^n(w)) \notin \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}}) \text{ for all } w\in [1:2^{nR}] \bigg| \rv{Y}^n=y^n} \pmf{\rv{Y}^n}(y^n) \\
    &= \sum_{y^n \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}})} \Prob{(y^n,\rv{Z}^n(w)) \notin \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}}) \text{ for all } w\in [1:2^{nR}] \bigg| \rv{Y}^n=y^n} \pmf{\rv{Y}^n}(y^n) \\
    &= \sum_{y^n \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}})} \prod_{w=1}^{2^{nR}} \Prob{(y^n,\rv{Z}^n(w)) \notin \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}}) } \pmf{\rv{Y}^n}(y^n) \\
    &= \sum_{y^n \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}})} \left( \Prob{(y^n,\rv{Z}^n(1)) \notin \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}}) } \right)^{2^{nR}} \pmf{\rv{Y}^n}(y^n).
\end{align}
Since $y^n \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}})$ and $\rv{Z}^n(1) \sim \prod_{i=1}^n \pmf{\rv{Z}} (z_i)$ it follows by the joint typicality lemma \cite[Ch. 2.5]{gamal2011} that for $n$ sufficiently large
\begin{equation}
    \Prob{(y^n,\rv{Z}^n(1)) \in \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}}) }  \geq 2^{-n(I(\rv{Y};\rv{Z}) + \delta(\epsilon))},
\end{equation}
where $\delta(\epsilon)$ tends to zero as $\epsilon \rightarrow 0$. Since $(1-x)^k \leq e^{-kx}$ for $x \in [0,1]$ and $k>0$, we have
\begin{align}
    \sum_{y^n \in \set{T}_{\epsilon'}^{(n)}(\pmf{\rv{Y}})} \left( \Prob{(y^n,\rv{Z}^n(1)) \notin \set{T}_{\epsilon}^{(n)}(\pmf{\rv{Y}\rv{Z}}) } \right)^{2^{nR}}
    & \leq  \left(1 - 2^{-n(I(\rv{Y};\rv{Z}) + \delta(\epsilon))} \right)^{2^{nR}} \\
    & \leq  e^{-2^{-n(I(\rv{Y};\rv{Z})-R + \delta(\epsilon))}}
\end{align}
which tends to zero as $n \rightarrow \infty$ if $R > I(\rv{Y};\rv{Z}) + \delta(\epsilon)$.

Define the ``typical distortion error" event
\begin{equation}
    \set{E}_d = \{ (\rv{X}^n, \rv{Y}^n, \rv{Z}^n(\rv{W})) \notin \set{T}_{\epsilon_d}^{(n)}(\pmf{\rv{X} \rv{Y}\rv{Z}}) \} \cap \event{E}^c.
\end{equation}
By Markov lemma \cite[Lemma 12.1]{gamal2011}, $\lim_{n\rightarrow \infty} \Prob{\event{E}_d} = 0$.
Now, by the law of total expectation and the typical average lemma,
\begin{align}
    \Exp[\set{C},\rv{X}^n]{d(\rv{X}^n,\rv{Z}^n(\rv{W}))}
    &= \Prob{\event{E}_d} \Exp[\set{C},\rv{X}^n]{d(\rv{X}^n,\rv{Z}^n(\rv{W})) | \event{E}_d} + \Prob{\event{E}_d^c} \Exp[\set{C},\rv{X}^n]{d(\rv{X}^n,\rv{Z}^n(\rv{W})) | \event{E}_d^c} \\
    &\leq \Prob{\event{E}_d} d_{\max}  + \Prob{\event{E}^c} \Exp[\set{C},\rv{X}^n]{d(\rv{X}^n,\rv{Z}^n(\rv{W})) | \event{E}_d^c}
\end{align}
where $d_{\max} = \max_{(x,z)\in \set{X} \times \set{Z}} d(x,z)$.
Note that
\begin{equation}
    \Exp[\set{C},\rv{X}^n]{d(\rv{X}^n,\rv{Z}^n(\rv{W})) | \event{E}_d^c}
    = \sum_{(x^n,z^n) \in \typset{\epsilon}{n}(\pmf{\rv{X}\rv{Z}})} \pmf{\rv{X}^n \rv{Z}^n}(x^n,z^n) d(x^n,z^n).
\end{equation}
For every $(x^n,z^n) \in \typset{\epsilon_d}{n}(\pmf{\rv{X}\rv{Z}})$ we have
\begin{align}
    d(x^n,z^n)
    &= \frac{1}{n} \sum_{i=1}^n d(x_i,z_i) \\
    &= \sum_{(a,c) \in \set{X} \times \set{Z}} \pmf{\bv{x} \bv{z}}(a,c) d(a,c) \\
    &\leq (1+\epsilon_d) \sum_{(a,c) \in \set{X} \times \set{Z}} \pmf{\rv{X}\rv{Z}} (a,c) d(a,c) \\
    &= (1+\epsilon_d) \Exp{d(\rv{X},\rv{Z})} \leq  D.
\end{align}
Thus,
\begin{equation}
    \Exp[\set{C},\rv{X}^n]{d(\rv{X}^n,\rv{Z}^n(\rv{W})) | \event{E}_d^c} \leq D
\end{equation}
and
\begin{equation}
    \limsup_{n \rightarrow \infty} \Exp[\set{C},\rv{X}^n]{d(\rv{X}^n,\rv{Z}^n(\rv{W}))} \leq D.
\end{equation}

